How long, O Bayesian network, will I sample thee? A program analysis perspective on expected sampling times

Bayesian networks (BNs) are probabilistic graphical models for describing complex joint probability distributions. The main problem for BNs is inference: Determine the probability of an event given observed evidence. Since exact inference is often infeasible for large BNs, popular approximate inference methods rely on sampling. We study the problem of determining the expected time to obtain a single valid sample from a BN. To this end, we translate the BN together with observations into a probabilistic program. We provide proof rules that yield the exact expected runtime of this program in a fully automated fashion. We implemented our approach and successfully analyzed various real-world BNs taken from the Bayesian network repository.

==> coupon-collector-lemma.tex <==
The next lemma can reduce the effort of verifying that Equation~\ref{eqn:parametrized-loop-assumption} holds for some given program to syntactic reasoning.
%
%
%
\begin{lemma}
     \label{lem:extension-helper}
       Let $C \in \pgcl$ and $f \in \E$. If $\RelNewRule{f}{C}$, then
       %
       %
       %
       \begin{equation*}
              \ert{C}{f} ~{}={}~ \ert{C}{0} + \wp{C}{1} \cdot f~.
       \end{equation*}
       %
       %
       %
       In particular, if $C$ terminates almost--surely, then
       %
       %
       %
      \begin{equation*}
              \ert{C}{f} ~{}={}~ \ert{C}{0} + f~.
       \end{equation*}
\end{lemma}
%
%
%
\begin{proof}
We have
%
%
%
\begin{align*}
                \ert{C}{f} ~{}={}~& \ert{C}{0} + \wp{C}{f}
                \tag{by Theorem~\ref{thm:ert-wp}} \\
       ~{}={}~& \ert{C}{0} + \wp{C}{1 \cdot f} \\
       ~{}={}~& \ert{C}{0} + \wp{C}{1} \cdot f~.
       \tag{$\RelNewRule{f}{C}$, see Lemma~\ref{lem:newrule-main} and }
\end{align*}
%
%
%
If $C$ terminates almost--surely, we further have $\wp{C}{1} = 1$ and thus
%
%
%
\begin{align*}
       \ert{C}{f} ~{}={}~ \ert{C}{0} + f~.
\end{align*}
%
%
%
\end{proof} \par
%
%
%



==> coupon-collector.tex <==
% !TEX root = ./main.tex

\section{Extension of Proof Rule to Coupon Collector}
\label{sec:extensions}
\newcommand{\runC}[2]{\mathsf{rt}_P(#1,#2)}
\newcommand{\innerProg}{P(k,i)}
\newcommand{\outerProg}{C_P}
\newcommand{\outerBody}{C_\mathit{body}}
\newcommand{\couponProg}{C_\mathit{cp}}
\newcommand{\couponInner}{C_\mathit{in}}
\newcommand{\couponOuter}{C_\mathit{out}}
\newcommand{\couponInnerAssign}{\PASSIGN{i}{\mathtt{Unif}[1 \ldots N]}}
\newcommand{\couponInnerBody}{C_\mathit{in\_ body}}


So far we developed proof rules to compute expected runtimes of either $f$-i.i.d.\  --or universally i.i.d.\ loops and\cmcomment{What do we do with this section?}
showed how to apply them to compute expected sampling times of Bayesian networks. In this section we show how our rules can be applied to deal with expected runtimes of programs with a more
complicated structure such as nested loops. %going beyond our Bayesian Network Language.
In particular, we show how they can be applied to solve the well--known Coupon Collector's Problem.

We consider paramterized loops $\outerProg$ of the form 
%
%
%
%\begin{figure}[H]
\begin{align*}
       &\WHILE{x > 0}\\
       &       \qquad \innerProg; \\
       &       \qquad \COMPOSE{\COMPOSE{\ASSIGN{i}{1}}{\ASSIGN{k}{k+1}}}{\ASSIGN{x}{x-1}} \}~.
\end{align*}
%
%
%
%
\noindent
Here $\innerProg \in \pgcl$ is a program where no more variables than $k$ and $i$ occur. In every iteration program $\innerProg$ is executed, $i$ is set to $1$, variable $k$ is increased by $1$,
and variable $x$ is decreased by one. It is easy to see that the loop iterates $x$--times if it is executed, and that its expected runtime is mainly determined by the runtime of $\innerProg$.
An analysis of the above program's expected runtime yields the following theorem.
%
%
%
\begin{theorem}
       \label{thm:parametrized-loop-runtime}
       Let $\outerProg$ denote a program of the above form. Furthermore, assume
       %
       %
       %
       \begin{equation}
              \ert{\innerProg}{f[i/1, x/x-1, k/k+1]} ~{}={}~ \ert{\innerProg}{0} + f[i/1, x/x-1, k/k+1]
              \label{eqn:parametrized-loop-assumption}
       \end{equation}
       %
       %
       %
       holds. Then for the expected runtime of program $\outerProg$, we have
       %
       %
       %
       \begin{align*}
              \ert{\outerProg}{0} ~{}={}~ 1 + 4x + \sum_{l=0}^{x-1}  \iverson{l = 0} \cdot \ert{\innerProg}{0}
                                 + \iverson{l \neq 0} \cdot \ert{\innerProg}{0}[k/k+l, i/1]~.
       \end{align*}
       %
       %
       %
\end{theorem}
%
%
%
\begin{proof}
By providing an $\omega$--invariant. See Appendix~\ref{proof-thm:parametrized-loop-runtime}.
\qed
\end{proof}
\noindent
%Wahrschl weg von hier \\
%Thus the expected runtime $\ert{\innerProg}{0}$ of program
%$\innerProg$ is a function parameterized by $k$ and $i$. We denote this runtime by $\runC{k}{i} \in \E$. Moreover, we assume that
%
%
%\begin{align}
%                      \ert{\innerProg}{f[i/1, x/x-1, k/k+1]} &~{}={}~ \ert{\innerProg}{0} + f[i/1, x/x-1, k/k+1] 
%                       \notag \\
%       &~{}={}~ \runC{k}{i} + f[i/1, x/x-1, k/k+1] \label{eqn:extension-assumption}
%\end{align}
%
%
%holds for all $f \in \E$. We want to analyze the expected runtime of program $\outerProg$ under the presented assumptions. 
%To this end, we propose the following as both a lower and upper $\omega$-invariant of program $\outerProg$ w.r.t.\ postruntime $0$:
%bis hier \\
%
%
%
%
%
%
%
%
%
%
%
%Since verifying that Equation~\ref{eqn:extension-assumption} holds might be somewhat involved, we propose the following lemma which can simplify the procedure.
%
%
%
Thus if we are able to determine $\ert{\innerProg}{0}$, the above theorem yields the expected runtime of the entire program.

Combining this theorem with the proof rules for i.i.d.\ loops yields a systematic technique to compute expected runtimes of more complicated programs which allows, for instance, to solve
the Coupon Collector's problem: Suppose
each box of cereal contains one of $N$ different coupons and once one has collected at least one coupon of each type, they can be traded for a prize. 
We want to determine the average number of boxes one has to buy until all coupons are collected under the assumption that the coupons are distributed uniformly.
The problem can be modeled by the following program $\couponProg$. 
%
%
%
\begin{align*}
       &\COMPOSE{\COMPOSE{\ASSIGN{k}{0}}{\ASSIGN{i}{1}}}{\ASSIGN{x}{N}}; \\
       &\WHILE{x>0} \\
       &\qquad \WHILE{i \leq k}\\
       &\qquad \qquad  \couponInnerAssign \}; \\
       &\qquad \COMPOSE{\COMPOSE{\ASSIGN{i}{1}}{\ASSIGN{k}{k+1}}}{\ASSIGN{x}{x-1}} \}
\end{align*} 
%
%
%
Observe that the outer loop (denoted by $\couponOuter$) of program $\couponProg$ is an instance of program $\outerProg$ where $\innerProg$ 
is instantiated with the inner loop, which we denote by $\couponInner$. It can be easily shown that loop $\couponInner$ is fulfills the premises of Theorem~\ref{thm:newrule-proof-rule}.
We thus immediately obtain
%
%
%
\begin{align}
               \ert{\couponInner}{0}
       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}~.          
                            \label{eqn:extension-runtime-inner-loop-0}
\end{align}
%
%
%
Moreover, it is straightforward to show that Equation~\ref{eqn:parametrized-loop-assumption} holds.
Hence Theorem~\ref{thm:parametrized-loop-runtime} is applicable and we obtain
%
%
%
%
%
%
\begin{align}
                 \ert{\couponProg}{0} 
        ~{}={}~& \ert{\couponOuter}{0}[k/0,i/1,x/N] 
                      \notag   \\
        ~{}={}~& 1 + 5N + \sum_{l=0}^{N-1}  \iverson{l = 0} \cdot  \left(\frac{2 \cdot \iverson{1 \leq 0}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq 0}} \right)          
                                   + \iverson{l \neq 0} \cdot   \left(\frac{2 \cdot \iverson{1 \leq l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq l}} \right) 
                         \tag{by Theorem~\ref{thm:parametrized-loop-runtime} and Equation~\ref{eqn:extension-runtime-inner-loop-0}} \\
        \eeq& \cdots \eeq 1 + N \cdot \left(5 + 2 \cdot \mathcal{H}_{N-1} \right)~,    
         \label{eqn:coupoun-harmonic-calculation}
\end{align}
%
%
%
where $\mathcal{H}_{N-1} = \sfrac{1}{1} + \sfrac{1}{2} +
\sfrac{1}{3} + \cdots + \sfrac{1}{N-1}$ denotes the $(N{-}1)$-st harmonic
number. For a complete calculation, % of Equation~\ref{eqn:coupoun-harmonic-calculation}
see Appendix~\ref{appendix:coupoun-harmonic-calculation}. Since the harmonic numbers approach asymptotically to the natural
logarithm, we conclude that the coupon collector algorithm $\couponProg$ runs in expected time $\Theta(N \cdot \log(N))$.





















%In order to analyze the expected runtime of loop $\couponOuter$, 
%we have to determine the expected runtime of $\couponInner$ 


%\kbcommentinline{weg von hier}
%and need to verify that Equation~\ref{eqn:extension-assumption} holds. Let $\couponInnerBody$ denote the body of loop $\couponInner$.
%First, we observe that loop $\couponInner$ is i.i.d.\ with respect to every 
%post-expectation $f \in \E$, because it holds that both
%
%
%\begin{enumerate}
%        \item $\wp{\couponInnerBody}{\iverson{i \leq k}} = \RelNewRule{ \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}{\couponInnerBody}$ and
%        \item $\wp{\couponInnerBody}{\iverson{i > k} \cdot f} = \RelNewRule{ \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \cdot f[i/j]}{\couponInnerBody}$ , 
%\end{enumerate}
%i.e.\ no variable occurring on the left-hand side of and assignment in $\couponInner$ also occurs in
%$\wp{\couponInnerBody}{\iverson{i \leq k}}$ or $\wp{\couponInnerBody}{\iverson{i > k} \cdot f}$. Moreover, we have 
%$\ert{\couponInnerBody}{0} = \RelNewRule{1}{\couponInnerBody}$. Hence Theorem~\ref{thm:newrule-proof-rule} yields
%
%
%
%\begin{align}
%                   &\ert{\couponInner}{f} \notag \\
%       ~{}={}~& 1 + \frac{\iverson{i \leq k}}{1 - \wp{\couponInnerBody}{\iverson{i \leq k}}} 
%                             \cdot \left(1 + \ert{\couponInnerBody}{0} + \wp{\couponInnerBody}{\iverson{i > k} \cdot f} \right) 
%                           + [i >k] \cdot f \notag \\
%       ~{}={}~& 1 + \frac{\iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}                 
%                             \cdot \left(2 +  \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \cdot f[i/j] \right) 
%                            + [i >k] \cdot f~. \label{eqn:extension-runtime-inner-loop-f}
%\end{align}
%
%
%
%In particular, we have
%
%
%
%\begin{align}
%                   \ert{\couponInner}{0}
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}~.          
%                            \label{eqn:extension-runtime-inner-loop-0}
%\end{align}
%
%
%
%Since $\RelNewRule{\couponInner}{f[i/1, x/x-1, k/k+1]}$, Lemma~\ref{lem:extension-helper} implies that Equation~\ref{eqn:extension-assumption} holds.
%
%
%
%\begin{align*}
%                   &\ert{\couponInner}{f[i/1, x/x-1, k/k+1]} \\
%      ~{}={}~& 1 + \frac{\iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}                 
%                           \cdot \left(2 + \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \cdot f[i/1, x/x-1, k/k+1] \right) 
%                            + [i >k] \cdot f \\
%       ~{}={}~& 1 + \frac{\iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}                 
%                             \cdot \left(2 + f[i/1, x/x-1, k/k+1] \cdot  \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k}\right) 
%                            + [i >k] \cdot f[i/1, x/x-1, k/k+1] 
%                            \tag{$j$ does not occur in $f[i/1, x/x-1, k/k+1]$}  \\
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}  
%                        + \frac{\iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}} 
%                                   \cdot  f[i/1, x/x-1, k/k+1] \cdot  \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \\      
%                   &\quad     + [i >k] \cdot f[i/1, x/x-1, k/k+1] \tag{multiply out}  \\
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}  
%                        + \frac{\iverson{i \leq k}}{\frac{1}{N} \cdot \left( N -  \sum_{j=1}^{N} \iverson{j \leq k} \right)} 
%                                   \cdot  f[i/1, x/x-1, k/k+1] \cdot  \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \\      
%                   &\quad     + [i >k] \cdot f[i/1, x/x-1, k/k+1]  \\
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}  
%                        + \frac{N \cdot \iverson{i \leq k}}{\sum_{j=1}^{N} \iverson{j > k} } 
%                                   \cdot  f[i/1, x/x-1, k/k+1] \cdot  \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j > k} \\      
%                   &\quad     + [i >k] \cdot f[i/1, x/x-1, k/k+1]
%                   \tag{$ N -  \sum_{j=1}^{N} \iverson{j \leq k} = \sum_{j=1}^{N} \iverson{j > k}$} \\
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}  
%                        + \iverson{i \leq k} \cdot  f[i/1, x/x-1, k/k+1] + [i >k] \cdot f[i/1, x/x-1, k/k+1] \\
%       ~{}={}~& 1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}}  
%                        + f[i/1, x/x-1, k/k+1]         
%                        \tag{$\iverson{i \leq k} + \iverson{i > k} = 1$}  \\
%       ~{}={}~& \ert{\couponInner}{0} + f[i/1, x/x-1, k/k+1] 
%                    \tag{by Equation~\ref{eqn:extension-runtime-inner-loop-0}}
%\end{align*}
%
%
%
%Thus we can apply Equation~\ref{eqn:extension-runtime-of-Cp} and obtain
%
%
%
%\begin{align*}
%                   &\ert{\couponOuter}{0} \\
%        ~{}={}~& 1 + 4x + \sum_{l=0}^{x-1}  \iverson{l = 0} \cdot \ert{\couponInner}{0}
%                                  + \iverson{l \neq 0} \cdot \ert{\couponInner}{0}[k/k+l, i/1] \\
%        ~{}={}~& 1 + 4x + \sum_{l=0}^{x-1}  \iverson{l = 0} \cdot  \left(1 + \frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}} \right)          
%                                   + \iverson{l \neq 0} \cdot   \left(1 + \frac{2 \cdot \iverson{1 \leq k+l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k+l}} \right)   \\
%        ~{}={}~& 1 + 5x + \sum_{l=0}^{x-1}  \iverson{l = 0} \cdot  \left(\frac{2 \cdot \iverson{i \leq k}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k}} \right)          
%                                  + \iverson{l \neq 0} \cdot   \left(\frac{2 \cdot \iverson{1 \leq k+l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq k+l}} \right)                                                    
%\end{align*}
%
%
%
%Overall, we get
%
%
%
%\begin{align*}
%                     \ert{\couponProg}{0} 
%        ~{}={}~& \ert{\couponOuter}{0}[k/0,i/1,x/N] \\
%        ~{}={}~& 1 + 5N + \sum_{l=0}^{N-1}  \iverson{l = 0} \cdot  \left(\frac{2 \cdot \iverson{1 \leq 0}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq 0}} \right)          
%                                   + \iverson{l \neq 0} \cdot   \left(\frac{2 \cdot \iverson{1 \leq l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq l}} \right)  \\
%       ~{}={}~& 1 + 5N + \sum_{l=0}^{N-1}  \iverson{l \neq 0} \cdot   \left(\frac{2 \cdot \iverson{1 \leq l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq l}} \right) \\  
%       ~{}={}~& 1 + 5N + \sum_{l=1}^{N-1} \frac{2 \cdot \iverson{1 \leq l}}{1 - \frac{1}{N} \cdot  \sum_{j=1}^{N} \iverson{j \leq l}} \\
%        ~{}={}~& 1 + 5N + 2 \cdot \sum_{l=1}^{N-1} \frac{1}{1 - \frac{l}{N}}
%                       \tag{$\sum_{j=1}^{N} \iverson{j \leq l} = l$} \\ 
%        ~{}={}~& 1 + 5N + 2 \cdot \sum_{l=1}^{N-1} \frac{N}{N-l} \\     
%        ~{}={}~& 1 + 5N + 2N \cdot \sum_{l=1}^{N-1} \frac{1}{N-l} \\      
%        ~{}={}~& 1 + 5N + 2N \cdot \sum_{l=1}^{N-1} \frac{1}{l}
%                       \tag{sum reordering} \\   
%        ~{}={}~& 1 + N \cdot \left(5 + 2 \cdot \mathcal{H}_{N-1} \right)~,            
%\end{align*}
%
%
%
%where $\mathcal{H}_{N-1} = \sfrac{1}{1} + \sfrac{1}{2} +
%\sfrac{1}{3} + \cdots + \sfrac{1}{N-1}$ denotes the $(N{-}1)$-th harmonic
%number. Since the harmonic numbers approach asymptotically to the natural
%logarithm, we conclude that the coupon collector algorithm
%$\couponProg$ runs in expected time $\Theta(N \cdot \log(N))$.%


%\newcommand{\rejectionProg}{C_{\mathit{sample}}}
%\newcommand{\rejectionProgBody}{C_{\mathit{body}}}

%\cmcommentinline{
%Shall we use the example below together with our introduction of $f$-i.i.d. programs?
%I think it is nice, but does not fit somewhere else...
%}

%\begin{example}[Expected Runtime of Rejection Sampling]
%Suppose we want to sample a point within a circle with center $(5,5)$ and radius $r=5$ uniformly at 
%random. We do so by means of rejection sampling, i.e.\ we sample a point within the square with
%center $(5,5)$ and side length $10$ uniformly at random and discard every point which is not located within the circle.
%\kbcomment{We could place some Tikz picture here (?)}
%The following probabilistic program $\rejectionProg$ models the procedure: \\
%
%
%
%\begin{align*}
%       & \WHILE{(x-5)^2 + (y-5)^2 \geq 25} \\
%       & \qquad \PASSIGN{x}{\mathtt{Unif}[0\ldots 10]}; \\
%       & \qquad \PASSIGN{y}{\mathtt{Unif}[0\ldots 10]}; \\ 
%       & \}
%\end{align*} \\
%
%
%
%In each iteration, we sample a point $(x,y) \in \{0, \ldots, 10 \}^2$ within the square. The loop guard ensures that we 
%obtain a point located within the circle when the loop terminates, since such a point $(x,y)$ satisfies the equation 
%(x-5)^2 + (y-5)^2 < 5^2$ and every point not satisfying this equation is discarded. The expected runtime of program 
%\rejectionProg$ corresponds to the average number of guard evaluations and samples necessary to obtain a point located
%within the circle using rejection sampling. Applying Theorem~\ref{thm:newrule-proof-rule} offers a very systematic 
%and mechanized technique to compute this runtime. In order to compute $\ert{\rejectionProg}{0}$ by applying 
%Theorem~\ref{thm:newrule-proof-rule}, we first need to check whether the loop is $0$-i.i.d. 
%For that, let $\rejectionProgBody$ denote the body of loop $\rejectionProg$. We have
%
%
%
%\begin{align*}
%       \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}} ~{}={}~ 
%       \frac{1}{121} \sum_{i=0}^{10} \sum_{j=0}^{10}
%                    \iverson{(i-5)^2 + (j-5)^2 \geq 25}
%       ~{}={}~\RelNewRule{\frac{48}{121}}{\rejectionProgBody}
%       \tag{by Table~\ref{table:wp}}
%\end{align*}
%
%
%
%and 
%
%
%
%\begin{align*}
%        \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 < 25} \cdot 0} ~{}={}~ 
%        \wp{\rejectionProgBody}{0} ~{}={}~ \RelNewRule{0}{\rejectionProgBody}~.
%        \tag{by strictness, see Theorem~\ref{thm:basic-prop}~(\ref{thm:basic-prop-strictness})}
%\end{align*}
%
%
%
%Moreover, we have $\ert{\rejectionProgBody}{0} = \RelNewRule{2}{\rejectionProgBody}$ and 
%$\wp{\rejectionProgBody}{1}=1$ since every loop--free program satisfies this property \kbcomment{shall we state this anywhere in some porperty--of--wp--theorem?}. 
%Hence Theorem~\ref{thm:newrule-proof-rule} is applicable and yields
%
%
%
%\begin{align*}
%                \ert{\rejectionProg}{0} 
%       &~{}={}~ \ert{\WHILEDO{(x-5)^2 + (y-5)^2 \geq 25}{\rejectionProgBody}}{0} \\
%       &~{}={}~ 1 + \frac{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}{1-\wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}}
%                    \cdot \left(1 + \ert{\rejectionProgBody}{0} \right) \\
%       &~{}={}~ 1 + \frac{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}{1-\frac{48}{121}}
%                    \cdot 3 \\
%       &~{}={}~ 1 + \iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \frac{363}{73}~.               
%\end{align*}
%
%
%
%Hence we require $1 + \sfrac{363}{73} \approx 5.973$ guard evaluations on average to sample a
%point within the circle uniformly at random using the rejection sampling method.
%\end{example}

%\begin{tikzpicture}

%\draw[help lines, use as bounding box, white] (-1, -1) grid (11, 11);

% x axis
%\draw[->, thick] (0, 0) -- (11, 0);
%\draw[->, thick] (0, 0) -- (0, 11);

%\foreach \x in {1, 2, ..., 10} {
%	\draw (\x, -0.1) -- (\x, 0.1);
%	\node at (\x, -0.3) {$\x$};
%}
%\foreach \y in {1, 2, ..., 10} {
%	\draw (-0.1, \y) -- (0.1, \y);
%	\node at (-0.3, \y) {$\y$};
%}


%\draw[thick, fill=shadegray] (0,0) -- (10,0) -- (10,10) -- (0,10) -- (0,0);
%\draw[thick, fill=white] (5,5) circle (5cm);


%\end{tikzpicture}



==> ert-rules.tex <==
% !TEX root = ./main.tex

\section{Runtimes of Independent and Identically Distributed Loops}
\label{sec:ert-rules}

\newcommand{\kGuard}{\varphi} % I introduce this macro because i am not sure which symbols we ue for guards
\newcommand{\kGuardB}{\iverson{\kGuard}}
\newcommand{\nkGuardB}{\iverson{\neg \kGuard}}
\newcommand{\exampleLoop}{C_{\mathit{flip}}}
%
%
\newcommand{\rejectionProg}{C_{\mathit{circle}}}
\newcommand{\rejectionProgBody}{C_{\mathit{body}}}
%
%
\noindent
We derive two proof rules that allow to systematically compute expected runtimes of \emph{independent and identically distributed 
loops} (or \emph{i.i.d.\ loops} for short). Intuitively, a loop is i.i.d.\ if the distributions of states reached at the end of the different loop iterations are equal.  
This is the case whenever there is no data flow across different iterations. 
In the non--probabilistic case, these loops either terminate after one iteration or never terminate at all. 
However, this is different for probabilistic programs. 
The class of probabilistic i.i.d.\ loops covers interesting applications.
As a running example, consider the program $\rejectionProg$ in Figure~\ref{fig:circle-loop}.
%as an example which we will consider frequently in the remainder of this section to clarify concepts. \\
%First, the random variables ``loop guard $\kGuard$ evaluates to true after iteration $i$" are independent and identically distributed.
%More formally, this means that $\wp{C}{\kGuardB}(\sigma)$ yields the probability of the guard evaluating $\true$ after \emph{one} iteration on input $\sigma$ 
%and thus $\wp{C}{\kGuardB}(\sigma)^i$ is the probability of the guard evaluating to $\true$ $i$--times in a row.
%Second, the expected runtime of the loop body doesn't alter through the different iterations, i.e.\ every iteration has the same expected runtime.
%Consider the following simple i.i.d.\ loop $C_{iid}$ as an example: \\
%
%
%
%\begin{align*}
%       &\WHILE{x = 0} \\
%       &\qquad \PASSIGN{x}{\frac{1}{2} \cdot \langle 0 \rangle + \frac{1}{2} \cdot \langle 1 \rangle} \\
%       &\}
%\end{align*} \\
%
%
%
%In each iteration we flip a fair coin and as long as we observe $x=0$, we flip the coin again. It is easy to see that there is no dataflow across the different iterations,
%because whenever variable $x$ is set, its value is never read in a subsequent iteration.  
\begin{figure}[t]
\begin{center}
\begin{minipage}{0.40\textwidth}
       \begin{align*}
              & \WHILE{(x-5)^2 + (y-5)^2 \geq 25} \\
              & \qquad \PASSIGN{x}{\mathtt{Unif}[0\ldots 10]}; \\
              & \qquad \PASSIGN{y}{\mathtt{Unif}[0\ldots 10]} \\ 
              & \}
       \end{align*} 
\end{minipage}
\qquad
\begin{minipage}{0.4\textwidth}
\begin{center}
\scalebox{1}{
\begin{tikzpicture}[scale=.3]

\draw[help lines, use as bounding box, white] (-1, -1) grid (11, 11);


% x axis
\draw[->, thick] (-0.3, 0) -- (11, 0);
\draw[->, thick] (0, -0.3) -- (0, 11);

\foreach \x in {1, 2, ..., 10} {
	\draw (\x, -0.3) -- (\x, 0.3);
}
\node at (5, -0.7) {\scriptsize $5$};
\node at (10, -0.7) {\scriptsize $10$};
\foreach \y in {1, 2, ..., 10} {
	\draw (-0.3, \y) -- (0.3, \y);
}
\node at (-0.8, 5) {\scriptsize $5$};
\node at (-0.8, 10) {\scriptsize $10$};


\draw[thick, fill=gray!20] (0,0) -- (10,0) -- (10,10) -- (0,10) -- (0,0);
\draw[thick, fill=white] (5,5) circle (5cm);



\node at (0.9, 0.9) {\scriptsize $\times$};
\node at (0.7, 1.8) {\scriptsize $\times$};

\node at (6, 7) {\scriptsize $\times$};
\node at (2.3, 3.5) {\scriptsize $\times$};
\node at (7.1, 2.1) {\scriptsize $\times$};
\node at (2, 7.5) {\scriptsize $\times$};
\node at (6.4, 8.3) {\scriptsize $\times$};
\node at (2, 7.5) {\scriptsize $\times$};
\node at (8.4, 4.5) {\scriptsize $\times$};
\node at (5.1, 4.9) {\scriptsize $\times$};
\node at (8.9, 3.5) {\scriptsize $\times$};


\node at (9.5, 9.1) {\scriptsize $\times$};
\node at (9.2, 9.3) {\scriptsize $\times$};

\node at (0.5, 9.3) {\scriptsize $\times$};

\node at (9, 0.8) {\scriptsize $\times$};
\node at (2, 7.5) {\scriptsize $\times$};
\node at (8.2, 0.3) {\scriptsize $\times$};
\node at (9.2, 1.1) {\scriptsize $\times$};
\end{tikzpicture}
}
\end{center}
\end{minipage} 
\end{center}
\caption{An i.i.d.\ loop sampling a point within a circle uniformly at random using rejection sampling. 
The picture on the right--hand side visualizes the procedure: 
In each iteration a point ($\times$) is sampled.
If we obtain a point within the white area inside the square, we terminate. 
Otherwise, i.e.\ if we obtain a point within the gray area outside the square, we resample.}
\label{fig:circle-loop}
\end{figure}
%
$\rejectionProg$ samples a point within a circle with center $(5,5)$ and radius $r=5$ uniformly at random using rejection sampling.
In each iteration, it samples a point $(x,y) \in \{0, \ldots, 10 \}^2$ within the square (with some fixed precision). 
The loop guard ensures that we resample whenever a sampled point is not located within the circle (white area).
%obtain a point located within the circle (white area) whenever the loop terminates, since such a point $(x,y)$ satisfies the equation 
%$(x-5)^2 + (y-5)^2 < 5^2$ and every point not satisfying this equation is discarded (gray area). 
Our proof rules allow to systematically compute the expected runtime of this loop, i.e. the average amount of probabilistic assignments and guard evaluations until a point within the circle is obtained.

We rely on existing proof rules originally presented in~\cite{DBLP:conf/esop/KaminskiKMO16} to establish the specialized rules presented in this paper.
%In order to establish the proof rules presented in this paper, we rely on proof rules presented in~\cite{DBLP:conf/esop/KaminskiKMO16}
%to reason about expected runtimes of loops. These rules build on the notion of $\omega$--invariants:
More precisely, we build on the notion of $\omega$--invariants:
%
%
%
\begin{theorem}[Expected Runtime Bounds from $\omega$-invariants~\textnormal{\cite{DBLP:conf/esop/KaminskiKMO16}}] \label{thm:omega-invariants}
	Let $C \in \pgcl$, $\kGuard$ be a guard, $f \in \E$, and $F_f$ be the \mbox{$\ertsymbol$--characteristic functional} of $\WHILEDO{\varphi}{C}$ with respect to postexpectation $f$.
	A sequence $\left(I_n\right)_{n \in \Nats}$ is called a lower $\omega$--invariant of $\WHILEDO{\kGuard}{C}$ with respect to~$f$,~iff
	%
	\begin{align*}
		I_0 \ppreceq F_f(0) 	\qand I_{n+1} \ppreceq F_f(I_n)~,
	\end{align*}
       %
       and $\left(I_n\right)_{n \in \Nats}$ is called an upper $\omega$--invariant of $\WHILEDO{\kGuard}{C}$ with respect to $f$, iff
	%
	\begin{align*}
		F_f(0) \ppreceq I_0 	\qand F_f(I_n) \ppreceq I_{n+1}~.
	\end{align*}
	%
	For lower and upper invariants the following holds:
       %
       \begin{enumerate}
              \item
                     If $I_n$ is a lower $\omega$-invariant of $\WHILEDO{\kGuard}{C}$ with respect to $f$ 
                    and $\lim_{n\to\infty} I_n$ exists \footnote{Limit $\lim_{n\to\infty} I_n$ is to be understood point-wise on 
                     $\Rposinf$, i.e.\ $\lim_{n\to\infty} I_n=\lambda\sigma. \lim_{n\to\infty}I_n(\sigma)$ 
                     and $\lim_{n\to\infty}I_n(\sigma)=\infty$ is considered a valid value.}, then
                     %
                     %             
                    \begin{equation*}
                           \lim_{n\to\infty} I_n \ppreceq  \ert{\WHILEDO{\kGuard}{C}}{f}~.
                    \end{equation*}
                    %
                    %
             \item 
                    If $I_n$ is an upper $\omega$-invariant of $\WHILEDO{\kGuard}{C}$ with 
                     respect to $f $ and $\lim_{n\to\infty} I_n$ exists, then
                     %
                     %
                    \begin{equation*}
                            \ert{\WHILEDO{\kGuard}{C}}{f} \ppreceq \lim_{n\to\infty} I_n ~.
                    \end{equation*}
                    %
                    %
        \end{enumerate}
        %
        %
\end{theorem}
%
%
%
Speaking intuitively, if $I_n$ is a lower (resp.\ upper) $\omega$--invariant of loop $\WHILEDO{\kGuard}{C}$, then 
$I_n$ yields a lower (resp.\ upper) bound on the expected runtime of those runs that finish within $n$ iterations. 
Bounds on the expected runtime of the entire loop are then obtained from the asymptotic behavior of $I_n$. 
Note that if $I_n$ is both a lower \emph{and} an upper $\omega$--invariant of loop $\WHILEDO{\kGuard}{C}$ w.r.t.\ postexpectation $f$ and $\lim_{n\to\infty} I_n$ exists, then 
%
%
%
\begin{equation*}
       \ert{\WHILEDO{\kGuard}{C}}{f} \eeq \lim_{n\to\infty} I_n~,
\end{equation*}
%
%
%
i.e.\ the asymptotic behavior of $I_n$, yields precisely the expected runtime of the loop with~respect~to~$f$.

A similar technique applies when reasoning about the $\wpsymbol$--semantics of loops. 
Instead of considering the entire loop, it is often useful to analyze its finite unrollings.
%
%
%
\begin{definition}[$n$--Unrolling of a Loop]
      \label{def:finite_approximations}
       Let $C \in \pgcl$ and $\kGuard$ be a guard. The \emph{$n$--unrolling} of a loop $\WHILEDO{\kGuard}{C}$, denoted $\WHILEDOapprox{\kGuard}{C}{n}$, is given
       by
       %
       %
       \begin{align*}
              \WHILEDOapprox{\kGuard}{C}{0} & \eeq  \DIVERGE \\
              \WHILEDOapprox{\kGuard}{C}{n+1} & \eeq  \ITE{\kGuard}{\COMPOSE{C}{ \WHILEDOapprox{\kGuard}{C}{n}}}{\SKIP}~. \tag*{$\triangle$}
       \end{align*}
       %
       %
\end{definition}
%
%
%
Given a loop $\WHILEDO{\kGuard}{C}$, program $\WHILEDOapprox{\kGuard}{C}{n}$ simulates that loop up to $n$ iterations. One can show that
%
%
%
\begin{equation*}
       \sup_{n \in \Nats}~\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq \wp{\WHILEDO{\kGuard}{C}}{f}~.
\end{equation*}
%
%
%
%Hence the supremum of the set $\left\{ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} ~\mid ~ n \in \Nats \right\}$ yields the $\wpsymbol$--semantics of the entire loop. 
%We make use of both the aforementioned fact and Theorem~\ref{thm:omega-invariants} in the remainder of this section. 
%
%
%

We now establish two proof rules for i.i.d. loops.
The correctness proof of both rules follows the same pattern: Assume we are given a loop $\WHILEDO{\kGuard}{C}$ and a postexpectation $f$.
By Theorem~\ref{thm:ert-wp}, we can split the expected runtime of the loop with respect to $f$ into
%
%
%
\begin{equation*}
       \ert{\WHILEDO{\kGuard}{C}}{f} ~{}={}~ \ert{\WHILEDO{\kGuard}{C}}{0} + \wp{\WHILEDO{\kGuard}{C}}{f}~.
\end{equation*}
%
%
%
Consequently, it suffices to determine $\ert{\WHILEDO{\kGuard}{C}}{0}$ and $\wp{\WHILEDO{\kGuard}{C}}{f}$. % in order to determine $\ert{\WHILEDO{\kGuard}{C}}{f}$.
We achieve the former by providing an $\omega$-invariant that captures the exact expected runtime of the loop and analyzing its asymptotic behavior.
For the latter case, we develop a theorem that provides a closed form of the $\wpsymbol$--semantics for all loops under consideration.
%by means of a theorem characterizing the 
%$\wpsymbol$--semantics of the loops in question  under consideration.
 %We start with analyzing what we call \emph{universally independent and identically distributed loops}.
\subsection{Universally Independent and Identically Distributed Loops}\label{sec:universally-iid}
%
%
%
Our first proof rule takes a global viewpoint on the i.i.d.\ property, i.e.\ it does not depend on a particular postexpectation.
Hence, we refer to loops within this class as \emph{universally i.i.d.\ loops}.
%
%
%
\begin{definition}[Universally i.i.d.\ Loops]
       \label{def:iid}
       Let $C$ be a $\pgcl$ program and $\kGuard$ be a guard. 
       We call a loop $\WHILEDO{\kGuard}{C}$ \emph{universally independent and identically distributed} (or \emph{universally i.i.d.} for short), iff for all $f \in \E$ it holds that
       \begin{equation*}
              \wp{C}{~\iverson{\kGuard} \cdot \wp{C}{f}~} \eeq  \wp{C}{\iverson{\kGuard}} \cdot \wp{C}{f}~.
              \tag*{$\triangle$}
       \end{equation*}
\end{definition}
%
%
%
This defines the i.i.d.\ property in a global manner. 
The intuition is the following:
No matter which postexpectation $f \in E$ we consider, the event that the guard evaluates to true (given by $\kGuardB$) shall be uncorrelated with the expected value of $f$ (given by $\wp{C}{f}$) after one loop iteration. 
We thus require
\begin{align*}
	\wp{C}{~\kGuardB \cdot \wp{C}{f}~} ~{}\stackrel{!}{=}{}~ &\wp{C}{\kGuardB} \cdot \wp{C}{\wp{C}{f}} \\
	\eeq & \wp{C}{\kGuardB} \cdot \wp{\COMPOSE{C}{C}}{f}~.
\end{align*} 
Furthermore, executing the loop body once or twice shall yield the same expected value for $f$.
We thus require
%
\begin{align*}
	\wp{C}{\kGuardB} \cdot \wp{\COMPOSE{C}{C}}{f} ~{}\stackrel{!}{=}{}~ \wp{C}{\kGuardB} \cdot \wp{C}{f}~.
\end{align*}
%
Taking these two requirements together results in the above definition.
%
%
%
\begin{example}
       \label{ex:universally-iid}
       As an example of a universally i.i.d.\ loop, consider the program in Figure~\ref{fig:circle-loop} (for some natural number $p \geq 1$ determining the precision of uniform sampling).
       To verify this, let $f \in \E$ be an expectation and let $\rejectionProgBody$
       denote the body of that loop. Then
       %
       %
       %
       \begin{align*}
              &\wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \wp{\rejectionProgBody}{f}} \\
              &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \frac{1}{121} \sum\limits_{i=0}^{10p} \sum\limits_{j=0}^{10 p} f[x/(\nicefrac i p), y/(\nicefrac j p)]}
                      \tag{Table~\ref{table:ert}} \\
                      &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}} \cdot \frac{1}{121} \sum\limits_{i=0}^{10p} \sum\limits_{j=0}^{10p} f[x/(\nicefrac i p), y/(\nicefrac j p)]
              \tag{$x$ \text{and} $y$ do not occur in $f[x/i, y/j]$} \\
              &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}} \cdot  \wp{\rejectionProgBody}{f}~.
              \tag*{$\triangle$}      
       \end{align*}
       %
       %
       %
\end{example}
%
%
%
\noindent
We now derive a characterization of the $\wpsymbol$--semantics of universally independent and identically distributed loops.
For that, we first analyze the $\wpsymbol$--semantics of their finite unrollings.
%
%
%
\begin{lemma}[$\wpsymbol$--Semantics of $n$--Unrollings of Universally I.I.D.\ Loops]
       \label{lem:oldrule_wp_finite_approximations}
       Let $C$ be a $\pgcl$ program and $\kGuard$ be a guard such that the loop 
       $\WHILEDO{\kGuard}{C}$ is universally i.i.d.
       Then, for all $n \in \Nats \setminus \{ 0 \}$ and $f \in \E$, we have
       %
       %
       \begin{align*}
              &\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} 
              \eeq  \iverson{\kGuard} \cdot \wp{C}{\iverson{\neg \kGuard} \cdot f}
               \cdot \left .\sum\limits_{i=0}^{n-2} \middle (\wp{C}{\iverson{\kGuard}}^i \right) + \iverson{\neg \kGuard} \cdot f~.
       \end{align*}
       %
       %
\end{lemma}
%
%
%
%
\begin{proof}
	By induction on $n$. See Appendix~\ref{proof-lem:oldrule_wp_finite_approximations}.
\end{proof}
\noindent
%
%
%
%
%Using Lemma~\ref{lem:oldrule_wp_finite_approximations}, 
This leads us to an exact characterization of expected outcomes of universally i.i.d.\ loops.
%we are now in a position to establish the following theorem.
%
%
%
\begin{theorem}[$\wpsymbol$--Semantics of universally i.i.d.\ Loops] \label{thm:oldrule-wpsemantics}
       Let $C \in \pgcl$ and let $\kGuard$ be a guard.
       If $\WHILEDO{\kGuard}{C}$ is universally i.i.d., then the following two statements hold for all $f \in \E$:
       \begin{enumerate}
              \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) < 1$ it holds that
                       \label{thm:oldrule-wpsemantics-one}
                       %
                       %
                       \begin{equation*}
                              \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                              \iverson{\kGuard}(\sigma) \cdot 
                              \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
                              + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) ~.
                       \end{equation*}
                       %
                       %
               \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) = 1$ it holds that
                        \label{thm:oldrule-wpsemantics-two}
                        %
                        %
                        \begin{equation*}
                        \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                        \nkGuardB (\sigma) \cdot f(\sigma) ~.
                        \end{equation*}
                        %
                        %
       \end{enumerate}
\end{theorem}
%
%
%\begin{proof}
%       The proof relies on the fact that
%       %
%       \begin{equation}
%              \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq 
%              \wp{\WHILEDO{\kGuard}{C}}{f}~,
%              \label{eq:in-proof:thm:oldrule-wpsemantics}
%       \end{equation}
%       %
%       which can easily be proven through showing by induction on $n$ that
%       %
%       \begin{align*}
%		\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq F_f^n(0)~,
%       \end{align*}
%       %
%       and then applying the Kleene Fixed Point Theorem.
%       %, which we omit here.
%       %
%       \autoref{eq:in-proof:thm:oldrule-wpsemantics} is equivalent to
%	   \begin{equation} \label{eqn:oldrule-continuity-states}
%       \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma)
%        \eeq  \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma)
%       \end{equation}
%       %
%       %
%       for all $\sigma \in \States$. 
%       
%       In order to prove the first statement of the theorem, suppose that $\wp{C}{\kGuardB}(\sigma) <1$.
%       We exploit the closed form of the geometric series,
%        i.e.\ 
%        \begin{align*}
%		\sum_{i=0}^{\omega} q  \eeq \frac{1}{1-q}~, \qquad \text{for } |q| <1~.
%        \end{align*}
%        Using this closed form, we calculate
%        %
%        %
%        \begin{align*}
%                 & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
%        & \eeq  \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
%                     \tag{by Equation \ref{eqn:oldrule-continuity-states}} \\
%                     %
%        & \eeq  \sup_{n \in \Nats}~
%                      \iverson{\kGuard}(\sigma) \cdot  \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
%                     \cdot \left. \sum\limits_{i=0}^{n-2} \middle( \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
%                    + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
%                    \tag{by Lemma \ref{lem:oldrule_wp_finite_approximations}} \\
%                    %
%        & \eeq   \iverson{\kGuard}(\sigma) \cdot \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
%                     \cdot \left. \sum\limits_{i=0}^{\omega} \middle( \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
%                    + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) \\
%                    %
%        & \eeq  \kGuardB (\sigma) \cdot 
%                     \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
%                     + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)~. \tag{closed form of geometric series}
%        \end{align*}
%        %
%        %
%        This proves the first statement of the theorem. 
%%        
%%        For the second statement of the theorem, suppose now that $\kGuardB(\sigma)=0$. 
%%        We then have
%%        %
%%        %
%%        \begin{align*}
%%                 & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
%%        & \eeq  \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
%%                     \tag{by Equation \ref{eqn:oldrule-continuity-states}} \\
%%        & \eeq  \sup_{n \in \Nats}~
%%                      \underbrace{\iverson{\kGuard}(\sigma)}_{{}={}0}
%%                      \cdot \left( \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
%%                      \cdot \sum\limits_{i=0}^{n-2} \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
%%                      + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
%%                      \tag{by Lemma \ref{lem:oldrule_wp_finite_approximations}} \\
%%        & \eeq  \sup_{n \in \Nats}~ \nkGuardB(\sigma) \cdot f(\sigma) \\
%%        & \eeq \nkGuardB(\sigma) \cdot f(\sigma)~.
%%        \end{align*}
%%        This proves the second statement of the theorem.
%%        %
%%        %
%
%%
%For the second statement of the theorem, suppose now that $\wp{C}{\iverson{\varphi}}(\sigma) = 1$.
%We observe that this can only be true if every state $\tau$ that is reachable with non--zero probability by executing $C$ on $\sigma$ has to satisfy $\varphi$. Otherwise, the integral would not add up to exactly 1.
%Formally,
%%
%\begin{align}
%	\wp{C}{\iverson{\varphi}}(\sigma) \eeq 1 \qiff \Exp{\Sigma}{\iverson{\varphi}}{\semantics{C}{\sigma}} = 1 \qiff \forall \semantics{C}{\sigma}(\tau) > 0 \implies \iverson{\varphi}(\tau) = 1
%	\label{eq:bennistheorem}
%\end{align}
%%
%From that, it follows that 
%%
%\begin{align*}
%	\wp{C}{\iverson{\neg \kGuard} \cdot f} (\sigma) \eeq \Exp{\Sigma}{\iverson{\neg \kGuard} \cdot f}{\semantics{C}{\sigma}} & \eeq \Exp{\Sigma}{f - \iverson{\kGuard} \cdot f}{\semantics{C}{\sigma}} \\
%	& \eeq \Exp{\Sigma}{f - 1 \cdot f}{\semantics{C}{\sigma}} \tag{by (\ref{eq:bennistheorem}) above} \\
%	& \eeq \Exp{\Sigma}{0}{\semantics{C}{\sigma}} \eeq 0
%\end{align*}
%%
%Now by Lemma~\ref{lem:oldrule_wp_finite_approximations}  and by $\wp{C}{\iverson{\neg \kGuard} \cdot f} (\sigma) = 0$ (see above) we get
%%
%\begin{align*}
%	\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} (\sigma) \eeq \iverson{\kGuard}(\sigma) \cdot 0 \cdot \left .\sum\limits_{i=0}^{n-2} \middle (\ldots \right) + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)  \eeq \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)
%\end{align*}
%%
%and thereby $\wp{\WHILEDO{\kGuard}{C}}{f} (\sigma) \eeq  \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)$.
%%
%%
%%
%\end{proof}
%
%
%
Verifying upper and lower bounds for expected values is a very involved task.
Verifying lower bounds is even more involved in practice than upper bounds.
It is thus worthwhile to note that the characterization of Theorem~\ref{thm:oldrule-wpsemantics} does not give us only bounds on the expected values, but instead we obtain the \emph{exact} expected values.

Building on this result, we next derive the exact expected runtimes of universally i.i.d.\ loops.
This requires a generalization of the universally i.i.d.\ property to a fixed number of loop iterations.
%$\WHILEDO{\kGuard}{C}$. This requires the next technical lemma.
%
%
%
\begin{lemma}
      \label{lem:oldrule-technical-three}
       Let $C \in \pgcl$ and $\kGuard$ be a guard.
       If $\WHILEDO{\kGuard}{C}$ is
       universally i.i.d., then the following equation holds for all $n \in \Nats$:
       %
       %
       \begin{equation*}
              \wp{C}{\kGuardB} \cdot \wp{C}{\kGuardB}^n \eeq 
              \wp{C}{\kGuardB \cdot \wp{C}{\kGuardB}^n}~.
       \end{equation*}
       %
       %
\end{lemma}
%
%
%
\begin{proof}
       By induction on $n$. See Appendix \ref{proof-lem:oldrule-technical-three}.
\end{proof}
\noindent
%
%
%
Intuitively, the above lemma ensures for every number of loop iterations $i$ that the events ``loop guard $\kGuard$ evaluates to $\true$ after 
iteration $i$" are independent and equally likely.\blkcomment{\atkb{} \atcm{} You say events here, but I see only one event. I do not get this intuition...}

In order to derive the expected runtime of a universally i.i.d.\ loop, we provide a lower and upper $\omega$--invariant with respect to postexpectation $0$
and analyze its asymptotic behavior.
Besides being universally i.i.d., such a loop has to satisfy two additional properties:
First, the loop body must terminate almost--surely, i.e.\ $\wp{C}{1} = 1$. 
Second, every iteration runs in the same expected time. 
This is formalized by $\wp{C}{\ert{C}{0}} = \ert{C}{0}$, because\blkcomment{This ``because" makes no sense to me : (} we have
%
%
%\begin{align*}
%                           & \wp{C}{\ert{C}{0}} ~{}={}~ \ert{C}{0} \\
%       {}\Longleftrightarrow{} & \wp{C}{\ert{C}{0}} + \ert{C}{0} ~{}={}~ \ert{C}{0} + \ert{C}{0} \\
%       {}\Longleftrightarrow{} & \ert{\COMPOSE{C}{C}}{0} ~{}={}~ 2 \cdot \ert{C}{0} ~.
%                             \tag{by Theorem~\ref{thm:ert-wp} and Table~\ref{table:wp}} 
%\end{align*}
\begin{align*}
                \ert{\COMPOSE{C}{C}}{0} &~{}={}~ \ert{C}{\ert{C}{0}} \tag{by Table~\ref{table:ert}} \\
       &~{}={}~ \ert{C}{0} + \wp{C}{\ert{C}{0}} \tag{by Theorem~\ref{thm:ert-wp}} \\
       &~{}={}~ \ert{C}{0} + \ert{C}{0} \\
       &~{}={}~ 2 \cdot \ert{C}{0}~.
\end{align*}
%
%
%
Thus, the expected runtime of two iterations is given by the expected runtime of one iteration multiplied by two. 
Notice, the fact that every iteration runs in the same \emph{expected time} does not necessarily imply that every iteration requires a fixed amount of time as the following example
demonstrates.
%
%
%
\begin{example}\label{ex:same-time}
       Consider the following $\pgcl$ program:
       %
       %
       %
       \begin{align*}
             &\WHILE{x \neq 0} \\
             &\qquad \PASSIGN{x}{\frac{1}{2} \cdot \langle 0 \rangle + \frac{1}{2} \cdot \langle 1 \rangle}; \\
             &\qquad \ITE{x=0}{\COMPOSE{\SKIP}{\SKIP}}{\SKIP} \}
       \end{align*}
       %
       %
       %
       In every iteration a fair coin is tossed and--dependent on the outcome--either two or one $\SKIP$ statements are executed.
       Even though it is almost--surely not the case that every iteration runs in exactly the same time, every iteration runs in the same \emph{expected time}, namely $3.5$. \hfill $\triangle$
\end{example}
\noindent
%
%
%
%
%Having the presented preliminaries at hand, 
We are now in a position to establish our first proof rule for computing expected runtimes. %for expected runtimes of universally i.i.d.\ loops.
\begin{theorem}[Proof Rule for Expected Runtimes of universally i.i.d.\ Loops]
       \label{thm:oldrule-proof-rule}
       Let $C$ be a $\pgcl$ program, $\kGuard$ be a guard, and $f \in E$. % be an arbitrary runtime. 
       Furthermore, assume the following conditions hold:
       %
       %
       \begin{enumerate}
              \item The loop $\WHILEDO{\kGuard}{C}$ is universally independent and identically distributed.
              \item The loop body terminates almost--surely, i.e. $\wp{C}{1} = 1$.
              \item Every iteration runs in the same \emph{expected} time, i.e. $\wp{C}{\ert{C}{0}} = \ert{C}{0}$.
       \end{enumerate}
       %
       %
       Then the expected runtime of the loop $\WHILEDO{\kGuard}{C}$ with respect to $f$ is given by:
       %
       %
       \begin{align*}
              & \ert{\WHILEDO{\kGuard}{C}}{f} \eeq 1+ \frac{\kGuardB \cdot \left(1 + \ert{C}{\nkGuardB \cdot f} \right)}{1- \wp{C}{\kGuardB}}  + \nkGuardB \cdot f~,
       \end{align*}
       %
       %
       where we define $\frac{0}{0} \coloneq 0$ and $\frac{a}{0} \coloneq \infty$ for $a \neq 0$.
\end{theorem}
%
%
%\begin{proof}
%       We show for every state $\sigma \in \States$ that
%       %
%       %
%       \begin{align*}
%              & \ert{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 1 + \frac{\kGuardB (\sigma) \cdot \left(1 + \ert{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)}  + \nkGuardB (\sigma) \cdot f (\sigma)~.
%        \end{align*}
%        %
%        %
%        To this end, we propose the following as both a lower and upper $\omega$--invariant of
%        the loop
%        % $\WHILEDO{\kGuard}{C}$ 
%        w.r.t.\ $0$:
%        %
%        %
%        %
%        \begin{equation}\label{eqn:oldrule-proof-rule-omega-invariant}
%              I_n = 1 + \kGuardB \cdot \left( \ert{C}{0} \cdot
%              \sum\limits_{i=0}^{n} \wp{C}{\kGuardB}^i ~+~ 
%              \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB}^i \right)
%       \end{equation}
%        %
%        %
%        %
%        For a verification that $I_n$ is indeed a lower and upper $\omega$--invariant, we refer to %the rigorous proof of this theorem located in 
%        Appendix~\ref{proof-thm_oldrule-proof-rule}.
%        %
%        %
%        %
%        We distinguish two cases for the probability of the loop guard being true after one exection of the loop body:
%        %We now consider the cases 
%        $\wp{C}{\kGuardB}(\sigma)<1$
%        and $\wp{C}{\kGuardB}(\sigma)=1$. 
%        %
%        %
%        \paragraph{Case $\wp{C}{\kGuardB}(\sigma)<1$:} 
%        %Theorem~\ref{thm:omega-invariants}, Equation~\ref{eqn:oldrule-proof-rule-omega-invariant},
%        %and the closed form of the geometric series yield
%        %
%        %
%        \begin{align}
%                         & \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) \notag \\
%                {}={}~& \lim_{n\to\infty} ~ \left( 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
%                             \sum\limits_{i=0}^{n} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
%                             \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB} (\sigma)^i \right) \right) 
%                             \tag{by Theorem~\ref{thm:omega-invariants} and  Equation~\ref{eqn:oldrule-proof-rule-omega-invariant}} \\
%                {}={}~& 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
%                             \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
%                             \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i \right) 
%                             \notag \\
%                 {}={}~& 1 + \kGuardB (\sigma) \cdot \left( 
%                               \frac{\ert{C}{0} (\sigma)}{1-\wp{C}{\kGuardB} (\sigma)} + 
%                                \frac{1}{1-\wp{C}{\kGuardB} (\sigma)} \right)      
%                                \tag{geometric series} \\
%                 {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 
%                               \ert{C}{0} (\sigma) + 1 \right)}{1-\wp{C}{\kGuardB} (\sigma)}~. 
%                               \label{eqn:oldrule-proof-caseone}                                                                    
%        \end{align}
%        %
%        %
%        Now, by Theorem~\ref{thm:ert-wp}, Theorem~\ref{thm:oldrule-wpsemantics}~(\ref{thm:oldrule-wpsemantics-one}), and Equation~\ref{eqn:oldrule-proof-caseone}, we obtain
%        %
%        %
%        \begin{align*}
%                         & \ert{\WHILEDO{\kGuard}{C}}{f} (\sigma) \\
%               {}={}~& \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) + \wp{\WHILEDO{\kGuard}{C}}{f} (\sigma)   
%                            \tag{by Theorem~\ref{thm:ert-wp}} \\
%               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 
%                            \ert{C}{0} (\sigma) + 1 \right)}{1-\wp{C}{\kGuardB} (\sigma)} +
%                            \iverson{\kGuard}(\sigma) \cdot 
%                            \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}  + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)
%                            \tag{by Theorem~\ref{thm:oldrule-wpsemantics}~(\ref{thm:oldrule-wpsemantics-one}) and Equation~\ref{eqn:oldrule-proof-caseone}} \\
%               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 1 + \ert{C}{0} (\sigma)
%                            + \wp{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)} 
%                             + \nkGuardB (\sigma) \cdot f (\sigma)\\
%               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 1 + \ert{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)}  + \nkGuardB (\sigma) \cdot f (\sigma)~. \tag{by Theorem~\ref{thm:ert-wp}}                                  
%        \end{align*}
%        %
%        %
%        
%        \paragraph{Case $\wp{C}{\kGuardB} (\sigma)=1$:} For a formal consideration of this case we again refer to Appendix~\ref{proof-thm_oldrule-proof-rule}. 
%        Intuitively, if $\wp{C}{\kGuardB} (\sigma)=1$, the loop guard is almost--surely true after an execution of the loop body on initial state $\sigma$.
%        Hence, the expected runtime of the loop is infinite if it is executed at least once.
%        Otherwise, it is $1$ due to the first (and only) guard evaluation.
%        %The reason is that $\wp{C}{\kGuardB} (\sigma)$ denotes the probability of the guard evaluating to $\true$ after one iteration on initial state $\sigma$. 
%        %That is, if
%        %$\wp{C}{\kGuardB} (\sigma) = 1$, then the guard evaluates to $\true$ after \emph{every} iteration.
%        %Here we provide a sketch:
%       % Since $\wp{C}{\kGuardB} (\sigma)$ denotes the probability of the loop guard evaluating to $\true$ after one iteration, $\wp{C}{\kGuardB} (\sigma)=1$
%       % implies that the guards evaluates to $\true$ after \emph{every} iteration. Thus, if the initial state satisfies the guard (i.e.\ $\kGuardB$).
%\end{proof}
%
%
%
%Let us demonstrate how Theorem~\ref{thm:oldrule-proof-rule} to a given i.i.d.\ loop in the next example.
%
%
%
%\newcommand{\exIIDLoop}{L}
%\newcommand{\exIIDLoopBody}{L_{\mathit{body}}}
%\begin{example}
%       Consider the following i.i.d.\ loop $\exIIDLoop$ and let $\exIIDLoopBody$ denote its body.
%       %
%       %
%       %
%       \begin{align*}
%              &\WHILE{i > 6} \\
%              &\qquad \PASSIGN{a_0, a_1, a_2}{\frac{1}{2} \cdot \langle 0 \rangle  + \frac{1}{2} \cdot \langle 1 \rangle}; \\
%              &\qquad \ASSIGN{i}{4a_2 + 2a_1 + a_0 + 1} \\
%              &\}
%       \end{align*}
%       %
%       %
%       %
%      The loop simulates a fair die by means of three fair toin cosses. We want to determine $\ert{L}{0}$, i.e. the average amount of guard evaluations and assignments necessary
%      to simulate the die, by applying Theorem~\ref{thm:oldrule-proof-rule}. We omit the calculations verifying that the premises of the theorem hold, which is relatively straightforward.
%      We have 
%       $\wp{\exIIDLoopBody}{\iverson{i > 6}} = \sfrac{1}{4}$ and $\ert{\exIIDLoopBody}{0} = 4$ due to the four assignments. Thus, we obtain
%       %
%      %
%      \begin{align*}
%                       &\ert{L}{0} \\
%                       &{}={}~ 1 + \frac{\iverson{i > 6}}{1 - \wp{\exIIDLoopBody}{\iverson{i > 6}}} \cdot \left(1 + \ert{\exIIDLoopBody}{0} \right)
%              ~{}={}~ 1 + \frac{\iverson{i > 6}}{1 - \sfrac{1}{4}} \cdot \left(1 + 4 \right) ~{}={}~ 1 + \iverson{i > 6} \cdot \frac{20}{3}~.
%       \end{align*}
%       %
%       %
%       %
%       Consequently, if $i > 6$ holds before the loop is executed, its expected runtime is  $1 + \sfrac{20}{3} \approx 7.67$. \hfill $\triangle$
%\end{example}
%
%
%
\begin{example}
        Let us determine the expected runtime of our running example --- the $\pgcl$ program $\rejectionProg$ from Figure~\ref{fig:circle-loop}. 
        We have already verified that $\rejectionProg$ is universally i.i.d.\ in Example~\ref{ex:universally-iid}. Since the loop body, denoted $\rejectionProgBody$, is loop--free,
        it holds that $\wp{\rejectionProgBody}{1}=1$. 
        Furthermore it is straightforward to verify that every iteration runs in the same expected time, i.e. $\wp{\rejectionProgBody}{\ert{\rejectionProgBody}{0}} = \ert{\rejectionProgBody}{0}$. 
        %Verifying this is straightforward and omitted here. 
        Consequently, Theorem~\ref{thm:oldrule-proof-rule} is applicable. 
        Hence,
        %
        %
        %
         \begin{align}\label{eqn:ex-universally-iid-runtime}
              \ert{\rejectionProg}{0}
              ~{}={}~ 1+ \frac{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \left(1 + \ert{\rejectionProgBody}{0} \right)}{1- \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}}~,
       \end{align}
        %
        %
        %
        where
        %
        %
        %
        \begin{equation*}
               \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}
              ~{}={}~ \frac{48}{121}
              \qquad \text{and} \qquad \ert{\rejectionProgBody}{0} ~{}={}~ 2~.
              \tag{by Table~\ref{table:wp} and Table~\ref{table:ert}}            
        \end{equation*}
        %
        %
        %
        By plugging the above values into Equation~\ref{eqn:ex-universally-iid-runtime}, we obtain the exact expected runtime of $\rejectionProg$:
        %
        %
        %
        \begin{equation*}
               \ert{\rejectionProg}{0} ~{}={}~ 1 + \iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \frac{363}{73}~. 
        \end{equation*}
        %
        %
        %
        Hence $1 + \sfrac{363}{73} \approx 5.97$ guard evaluations and random assignments are required on average to sample a
        point within the circle uniformly at random using the rejection sampling method.\hfill $\triangle$
\end{example}
%
%
%
\subsection{$\boldsymbol{f}$--Independent and Identically Distributed Loops}
%
%
%
Towards proof rules for expected outcomes and expected runtimes of probabilistic programs that, in principle, can be discharged and applied automatically,
we present a syntactical notion of the i.i.d.\ property.
%Similar to the previous section we subsequently develop suitable proof rules.
%In this subsection, we define the i.i.d.\ property in a more syntactic manner and derive another proof rule for loops satisfying this property.
While the proof rule presented in Section~\ref{sec:universally-iid} deals with loops being i.i.d.\ with respect to \emph{all} postexpectations, the proof rule presented in this
subsection only requires that the loop is i.i.d.\ with respect to a \emph{single} given postexpectation.
Our syntactical version of i.i.d.\ loops relies on the concept of expectations that are not affected by a $\pgcl$ program:
%More formally:
%
%
\begin{definition}
  Let $C$ be a $\pgcl$ program and $f \in \E$ be an expectation.
  Moreover, let $\VarsAssign{C}$ denote the set of all variables that are modified by $C$.
  That is, they occur on the left-hand side of an assignment in $C$.
  Analogously, let $\VarsInExp{f}$ be the set of all variables that occur in $f$, i.e.\ formally
  %
  \begin{align*}
  	x \in \VarsInExp{f} \qqiff \exists\, \sigma~ \exists\, v, v' \colon \quad f(\sigma\statesubst{x}{v}) \nneq f(\sigma\statesubst{x}{v'})~.
  \end{align*}
  %
  Then $f$ is \emph{unaffected} by $C$, denoted $\RelNewRule{f}{C}$, if and only if $\VarsInExp{f} \cap \VarsAssign{C} = \emptyset$. \hfill$\triangle$
\end{definition}
\noindent
%
%
%We first define a relation which is of importance for the results of this subsection.
%Given $C \in \pgcl$, let $\VarsAssign{C} \subseteq \Vars$
%denote the set of variables occurring at least once on the left-hand side of an assignment in $C$. Furthermore, given an expectation 
%$f \in E$, we let $\VarsInExp{f} \subseteq \Vars$ denote the set of variables that occur in $f$. 
%Relation ${\RelSymbolNewRule} \subseteq \E \times \pgcl$ is then defined by 
%$\RelNewRule{f}{C}$ iff $\VarsInExp{f} \cap \VarsAssign{C} = \emptyset$, i.e.\ $\RelNewRule{f}{C}$ holds iff no variable in $f$ occurs
%on the left-hand side of an assignment in $C$. 
%\noindent
%
The reason why we are interested in expectations that are unaffected by $\pgcl$ programs lies in a simple yet useful observation:
If $\RelNewRule{g}{C}$, then \emph{$g$ can be treated like a constant} with respect to the transformer $\wpsymbol$ (i.e.\ like the $r$ in Theorem~\ref{thm:basic-prop}~(\ref{thm:basic-prop-linearity})).
For our running  example $\rejectionProg$ (see Figure~\ref{fig:circle-loop}), the expectation $f = \wp{\rejectionProgBody}{\iverson{x + y \leq 10}}$ is unaffected by the loop body $\rejectionProgBody$ of $\rejectionProg$. Consequently, we have $\wp{\rejectionProgBody}{f} = f$.
In general, we obtain the following property.
%The next lemma states a crucial fact: 
%If $\RelNewRule{g}{C}$, then $g$ can be treated as a constant w.r.t.\ transformer $\wp{C}{\cdot}$.
%
%
%
\begin{lemma}[Scaling by Uneffected Expectations]
      \label{lem:newrule-main}
      Let $C$ be a $\pgcl$ program and let $f,g \in \E$.
      Then $\RelNewRule{g}{C}$ implies
      %
      %
      \begin{equation*}
             \wp{C}{g \cdot f} \eeq  g \cdot \wp{C}{f}~.
      \end{equation*}
      %
      %
\end{lemma}
%
%
%
\begin{proof}
By induction on the structure of $C$. See Appendix~\ref{proof-lem:newrule-main}.
\end{proof}
\noindent
%
%
%
Based on this observation, we define our second notion of i.i.d.\ loops.
%Consequently, a loop being i.i.d.\ with respect to a given postexpectation can be defined as follows:
%
%
%
\begin{definition}[$f$-Independent and Identically Distributed Loops]\label{def:f-iid}
       Let $C \in \pgcl$, $\kGuard$ be a guard, and $f \in E$. 
       Then we call the loop $\WHILEDO{\kGuard}{C}$
       \emph{$f$--independent and identically distributed (or $f$--i.i.d.) for short}, if both
       %
       %
       \begin{enumerate}
              \item $\RelNewRule{\wp{C}{\kGuardB}}{C}$, and \label{item:newrule-defidd-one}
              \item $\RelNewRule{\wp{C}{\nkGuardB \cdot f}}{C}$. \hfill $\triangle$ \label{item:newrule-defidd-two}
       \end{enumerate}
       %
       %
\end{definition}
\noindent
%
%
%
Intuitively, the first condition ensures that all events of the form "the loop guard $\kGuard$ evaluates to $\true$ after $i$ iterations" are independent and equally likely.\blkcomment{same here. do not get this}
Moreover, the event "the loop guard $\kGuard$ eventually evaluates to $\false$" should also be independent of the previous events.\blkcomment{this is not exactly what the second condition states}
This is required by the second condition.
%
%One can show that Condition~\ref{item:newrule-defidd-one} and Lemma~\ref{lem:newrule-main} imply $\wpFold{C}{\kGuardB}{\kGuardB}{n} = \wp{C}{\kGuardB}^{n+1}$.
%Speaking intuitively, this definition implies that the events ``loop guard $\kGuard$ evaluates to $\true$ after iteration $i$" are independent
%and equally likely. An intuition on Condition~\ref{item:newrule-defidd-two} can be given as follows:
%Expectation $\wp{C}{\nkGuardB \cdot f}$ yields the expected value of $f$ for those runs of $C$ for which the loop guard evaluates to $\false$.
% This expected value shall also be independent of the events ``loop guard $\kGuard$ evaluates to $\true$ after iteration $i$".
 %Indeed, one can show that Condition~\ref{item:newrule-defidd-one}, Condition~\ref{item:newrule-defidd-two}, and Lemma~\ref{lem:newrule-main} imply $\wpFold{C}{\wp{C}{\nkGuardB \cdot f}}{\kGuardB}{n} = \wp{C}{\kGuardB}^{n} \cdot \wp{C}{\nkGuardB \cdot f}$.
%
%
%
\begin{example}
        Our example program $\rejectionProg$ (see Figure~\ref{fig:circle-loop}) is $f$--i.i.d. for all $f \in \E$. 
        This is due to the fact that
       %
       %
       %
       \begin{equation*}
              \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}
              ~{}={}~ \RelNewRule{\frac{48}{121}}{\rejectionProgBody}
              \tag{by Table~\ref{table:wp}}
       \end{equation*}
       %
       %
       %
       and (again for some fixed precision $p \in \Nats \setminus \{0\}$)
       %
       %
       %
       \begin{align*}
             &\wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 > 25} \cdot f} \\
             &{}={}~ \RelNewRule{\frac{1}{121} \cdot \sum\limits_{i=0}^{10p}\sum\limits_{j=0}^{10p} \iverson{(\nicefrac i p -5)^2 + (\nicefrac j p -5)^2 > 25} \cdot f[x/(\nicefrac i p),y/(\nicefrac j p)]}{\rejectionProgBody}~.
             \tag*{$\triangle$}
       \end{align*}
       %
       %
       %
\end{example}
\noindent
%
%
The notion of $f$--i.i.d.\ loops has two benefits when compared to the notion of universally i.i.d.\ loops:
First, one can discharge whether a given loop in $\pgcl$ is an $f$--i.i.d.\ loop by purely syntactical checks.
Second, a loop does not have to be i.i.d.\ with respect to \emph{all} postexpectations.

However, \emph{both notions of i.i.d. loops are justified} as \emph{none of the two subsumes the other}.
Let us consider an example loop in $\pgcl$ that is an $f$--i.i.d.\ loop, but not a universally i.i.d.\ loop:
%
%This definition of i.i.d.\ loops has two advantages compared to Definition~\ref{def:iid} (universally i.i.d.\ loops). On the one hand, deciding whether a given loop is $f$--i.i.d.\ 
%consists mostly of syntactic reasoning in many cases. In particular, if the loop body is loop--free and if $f$ is given as an arithmetic expression over the program variables.
%On the other hand, the loop doesn't have to be i.i.d.\ with respect to \emph{all} postexpectations, which will allow us to compute 
%expected runtimes of loops like the following using the proof rule presented in this subsection:
%
%
%
\begin{align*}
        &\WHILE{x = 0} \\
        &\qquad \PASSIGN{x}{\frac{2}{5} \cdot \langle 0 \rangle + \frac{2}{5} \cdot \langle 1 \rangle + \frac{1}{5} \cdot \langle 2 \rangle}; \\
        &\qquad \ASSIGN{z}{z+1} \}
\end{align*}
%
%
%
The loop is not i.i.d.\ with respect to \emph{all} postexpectations: There is data flow across different loop iterations due to the counter $z$. 
Thus, Theorem~\ref{thm:oldrule-proof-rule} is not applicable in order to compute the expected runtime of this loop.
However, $z$ does not influence the probability of the guard evaluating to $\true$ after one iteration. Hence, this loop is $f$--i.i.d.\ for all postexpectations $f$
in which $z$ does not occur.

In contrast, there are loops for which Theorem~\ref{thm:oldrule-proof-rule} is applicable but no postexpectation $f$ exists such that the loop is $f$--i.i.d.
Consider, for instance, the loop
%
%
%
%\begin{align*}
%    &\WHILE{k \neq 1} \\
%    &\qquad \ASSIGN{k}{k+1}; \\
%    &\qquad \ASSIGN{k}{k-1} \\
%    &\}~.
%\end{align*}
\begin{align*}
       \WHILEDO{k \neq 1}{\COMPOSE{\ASSIGN{k}{k+1}}{\ASSIGN{k}{k-1}}}~.
\end{align*}
%
%
%
One can easily show that this loop is universally independent and identically distributed and that the proof rule for expected runtimes of universally i.i.d.\ loops is applicable. 
It is, however, not $f$--i.i.d. for any postexpectation $f$, because $\wp{\COMPOSE{\ASSIGN{k}{k+1}}{\ASSIGN{k}{k-1}}}{\iverson{k \neq 1}} = \iverson{k \neq 1}$ and $\iverson{k \neq 1}$ is clearly \emph{not unaffected} by $\COMPOSE{\ASSIGN{k}{k+1}}{\ASSIGN{k}{k-1}}$.
%, this loop cannot be 
%$f$--independent and identically distributed for any postexpectation $f$. 
%
%
%   \noindent
%Next, we establish a theorem characterizing the $\wpsymbol$--semantics of an $f$--i.i.d.\ loop.

To conclude this section, we establish proof rules for $f$--i.i.d.\ loops similar to the rules for universally i.i.d.\ loops (Section~\ref{sec:universally-iid}).
%
\begin{theorem}[$\wpsymbol$--Semantics of $f$--I.I.D.\ Loops] \label{thm:newrule-wpsemantics}
       Let $C \in \pgcl$, $\kGuard$ be a guard, and $f \in \E$.
       If the loop $\WHILEDO{\kGuard}{C}$ is $f$--i.i.d., then the following two statements hold:
       \begin{enumerate}
              \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) < 1$ it holds that
                       \label{thm:newrule-wpsemantics-one}
                       %
                       %
                       \begin{equation*}
                              \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                              \iverson{\kGuard}(\sigma) \cdot 
                              \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
                              + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) ~.
                       \end{equation*}
                       %
                       %
               \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) = 1$ it holds that
                        \label{thm:newrule-wpsemantics-two}
                        %
                        %
                        \begin{equation*}
                        \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                        \nkGuardB (\sigma) \cdot f(\sigma) ~.
                        \end{equation*}
                        %
                        %
       \end{enumerate}
\end{theorem}
%
%
\begin{proof}
       By analyzing the $\wpsymbol$--semantics of an $f$--i.i.d.\ loop's finite approximations, see Appendix~\ref{lem:newrule_wp_finite_approximations}.
       The proof is then analogous to the proof of Theorem~\ref{thm:oldrule-wpsemantics}.
       %The proof relies on a continuity argument\kbcomment{we need a quote here, don't we?}, namely 
       %
       %
       %\begin{equation*}
       %       \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq 
       %       \wp{\WHILEDO{\kGuard}{C}}{f}~,
       %\end{equation*}
       %
       %
       %which implies 
	   %\begin{equation} \label{eqn:newrule-continuity-states}
       %\sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma)
       % \eeq  \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma)
       %\end{equation}
       %
       %
       %for all $\sigma \in \States$. 
       %In order to prove the first statement, assume $\wp{C}{\kGuardB}(\sigma) <1$.
       %By making use of the closed form of the geometric series,
       % i.e.\ $\sum\limits_{i=0}^{\infty} q  = \frac{1}{1-q}$ for all $|q| <1$, we compute
        %
        %
       % \begin{align*}
       %          & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
       % {}={}~& \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
       %              \tag{by Equation \ref{eqn:newrule-continuity-states}} \\
       % {}={}~& \sup_{n \in \Nats}~
       %               \iverson{\kGuard}(\sigma) \cdot \left( \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
       %              \cdot \sum\limits_{i=0}^{n-2} \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
       %             + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
       %             \tag{by Lemma \ref{lem:newrule_wp_finite_approximations}} \\
       % {}={}~&  \iverson{\kGuard}(\sigma) \cdot \left( \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
       %              \cdot \sum\limits_{i=0}^{\infty} \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
       %             + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) \\
       % {}={}~& \kGuardB (\sigma) \cdot 
       %              \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
       %              + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)~. \tag{geometric series}
       % \end{align*}
        %
        %
       % This verifies the first statement. For the second statement now assume $\kGuardB(\sigma)=1$. 
       % We have
        %
        %
       % \begin{align*}
       %          & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
       % {}={}~& \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
       %              \tag{by Equation \ref{eqn:newrule-continuity-states}} \\
       % {}={}~& \sup_{n \in \Nats}~
       %               \underbrace{\iverson{\kGuard}(\sigma)}_{{}={}~0}
       %               \cdot \left( \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
       %               \cdot \sum\limits_{i=0}^{n-2} \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
       %               + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
       %               \tag{by Lemma \ref{lem:newrule_wp_finite_approximations}} \\
       % {}={}~& \sup_{n \in \Nats}~ \nkGuardB(\sigma) \cdot f(\sigma) = \nkGuardB(\sigma) \cdot f(\sigma)~.
       % \end{align*}
        %
        %
\end{proof}        
\noindent              
%
%
%
%In order to derive an $\omega$--invariant for a $0$--i.i.d.\ loop $\WHILEDO{\kGuard}{C}$,
%that loop has to fulfill two further properties besides being $0$--i.i.d.
%First, the loop body must terminate almost--surely, i.e. $\wp{C}{1} = 1$.
%Moreover, every iteration shall run in the same expected time formalized syntactically by $\RelNewRule{\ert{C}{0}}{C}$, because we then have
%
%
%
%\begin{align*}
%       \ert{\COMPOSE{C}{C}}{0} &~{}={}~ \ert{C}{\ert{C}{0}}
%       \tag{by Table~\ref{table:ert}} \\ 
%       &~{}={}~ \ert{C}{0} + \wp{C}{\ert{C}{0}} 
%       \tag{by Theorem~\ref{thm:ert-wp}} \\ 
%       &~{}={}~ \ert{C}{0} + \wp{C}{1 \cdot \ert{C}{0}} \\
%       &~{}={}~ \ert{C}{0} + \wp{C}{1} \cdot \ert{C}{0}
%       \tag{$\RelNewRule{\ert{C}{0}}{C}$, see Lemma~\ref{lem:newrule-main}} \\
%       &~{}={}~ 2 \cdot \ert{C}{0}~.
%       \tag{$\wp{C}{1}=1$}
%\end{align*}
%
%
%That is, the expected runtime of two iteration is given by the runtime of one iteration multiplied by two.
%Example~\ref{ex:same-time} provides a loop demonstrating that if every iteration runs in the same \emph{expected} time, this does not necessarily imply
%that every iteration requires a fixed amount of time.
%
%
%
%
%
%
%
%
We now derive a proof rule for the expected runtime of an $f$--i.i.d.\ loop $\WHILEDO{\kGuard}{C}$.
As it was the case for universally i.i.d.\ loops, those loops have to fulfill the same two additional properties:
The loop body must terminate almost--surely, i.e.\ $\wp{C}{1}=1$, and every iteration shall run in the same expected time, i.e.\ $\RelNewRule{\ert{C}{0}}{C}$.
%
%
%
\begin{theorem}[Proof Rule for Expected Runtimes of $f$--I.I.D.\ Loops]
       \label{thm:newrule-proof-rule}
       Let $C \in \pgcl$, $\kGuard$ be a guard, and $f \in E$ such that the following conditions hold:
       %
       %
       \begin{enumerate}
              \item Loop $\WHILEDO{\kGuard}{C}$ is $f$--i.i.d.
              \item $\wp{C}{1} = 1$ (loop body terminates almost--surely).
              \item $\RelNewRule{\ert{C}{0}}{C}$ (every iteration runs in the same expected time).
       \end{enumerate}
       %
       %
       Then for the expected runtime of the loop $\WHILEDO{\kGuard}{C}$ with respect to postruntime $f$ it holds
       that
       %
       %
       \begin{align*}
              &\ert{\WHILEDO{\kGuard}{C}}{f} \eeq 1+ \frac{\kGuardB \cdot \left(1 + \ert{C}{\nkGuardB \cdot f} \right)}{1- \wp{C}{\kGuardB}} + \nkGuardB \cdot f~,
       \end{align*}
       %
       %
       where $\frac{0}{0} \coloneq 0$ and $\frac{a}{0} \coloneq \infty$ for $a \neq 0$.
\end{theorem}
%
%
%
\begin{proof}
	By providing a lower and upper $\omega$--invariant w.r.t.\ postexpectation $0$ (see Appendix~\ref{lem:newrule-omega-invariant}) and making use of Theorem~\ref{thm:newrule-wpsemantics}.
	The proof is then analogous to the proof of 
	Theorem~\ref{thm:oldrule-proof-rule}.
       %We prove the theorem point-wise, i.e. we show that 
       %
       %
       %\begin{align*}
        %                   & \ert{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
         %     \eeq  & 1 + \frac{\kGuardB (\sigma)}{1- \wp{C}{\kGuardB} (\sigma)} 
          %                    \cdot \left(1 + \ert{C}{0} (\sigma)
        %                    + \wp{C}{\nkGuardB \cdot f} (\sigma) \right) + \nkGuardB (\sigma) \cdot f (\sigma)
        %\end{align*}
        %
        %
        %holds for every state $\sigma \in \States$. We distinguish the cases $\wp{C}{\kGuardB}(\sigma)<1$
        %and $\wp{C}{\kGuardB}(\sigma)=1$. 
        %
        %
        %\emph{Case $\wp{C}{\kGuardB}(\sigma)<1$:} Theorem~\ref{thm:omega-invariants}, Lemma \ref{lem:newrule-omega-invariant},
        %and the closed form of the geometric series yield
        %
        %
        %\begin{align}
        %                 & \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) \notag \\
        %        {}={}~& \lim_{n\to\infty} ~ \left( 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
        %                    \sum\limits_{i=0}^{n} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
        %                     \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB} (\sigma)^i \right) \right) 
        %                     \tag{by Theorem~\ref{thm:omega-invariants} and  Lemma~\ref{lem:newrule-omega-invariant}} \\
        %        {}={}~& 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
        %                     \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
        %                     \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i \right) 
        %                     \notag \\
        %         {}={}~& 1 + \kGuardB (\sigma) \cdot \left( 
        %                       \frac{\ert{C}{0} (\sigma)}{1-\wp{C}{\kGuardB} (\sigma)} + 
        %                        \frac{1}{1-\wp{C}{\kGuardB} (\sigma)} \right)      
        %                        \tag{geometric series} \\
        %         {}={}~& 1 + \frac{\kGuardB (\sigma)}{1-\wp{C}{\kGuardB} (\sigma)} \cdot \left( 
        %                       \ert{C}{0} (\sigma) + 1 \right)~. 
        %                       \label{eqn:newrule-proof-caseone}                                                                    
        %\end{align}
        %
        %
        %Now, by Theorem~\ref{thm:ert-wp}, Theorem~\ref{thm:newrule-wpsemantics}~(\ref{thm:newrule-wpsemantics-one}), and Equation~\ref{eqn:newrule-proof-caseone}, we obtain
        %
        %
        %\begin{align*}
        %                & \ert{\WHILEDO{\kGuard}{C}}{f} (\sigma) \\
        %       {}={}~& \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) + \wp{\WHILEDO{\kGuard}{C}}{f} (\sigma)   
        %                    \tag{by Theorem~\ref{thm:ert-wp}} \\
        %       {}={}~& 1 + \frac{\kGuardB (\sigma)}{1-\wp{C}{\kGuardB} (\sigma)} \cdot \left( 
        %                    \ert{C}{0} (\sigma) + 1 \right) +
        %                    \iverson{\kGuard}(\sigma) \cdot 
        %                    \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
        %                    + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)
        %                    \tag{by Theorem~\ref{thm:newrule-wpsemantics}~(\ref{thm:newrule-wpsemantics-one}) and Equation~\ref{eqn:newrule-proof-caseone}} \\
        %       {}={}~& 1 + \frac{\kGuardB (\sigma)}{1- \wp{C}{\kGuardB} (\sigma)} 
        %                    \cdot \left(1 + \ert{C}{0} (\sigma)
        %                    + \wp{C}{\nkGuardB \cdot f} (\sigma) \right) + \nkGuardB (\sigma) \cdot f (\sigma)~.                                  
        %\end{align*}
        %
        %
        %
        %\emph{Case $\wp{C}{\kGuardB} (\sigma)=1$:} We distinguish the cases $\kGuardB (\sigma) =0$ and $\kGuardB (\sigma)=1$.
        %First assume $\kGuardB (\sigma) =0$. Then from Theorem~\ref{thm:omega-invariants} and Lemma~\ref{lem:newrule-omega-invariant} it follows that
        %
        %
        %\begin{align}
        %       & \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) \notag \\
        %        {}={}~& \lim_{n\to\infty} ~ \left( 1 + \underbrace{\kGuardB (\sigma)}_{{}={}~0} \cdot \left( \ert{C}{0} (\sigma) \cdot
        %                     \sum\limits_{i=0}^{n} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
        %                     \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB} (\sigma)^i \right) \right) 
        %                     \tag{by Theorem~\ref{thm:omega-invariants} and  Lemma~\ref{lem:newrule-omega-invariant}} \\
        %        {}={}~& \lim_{n\to\infty} ~1 \eeq  1~. \label{eqn:newrule-proof-casetwo-one}            
        %\end{align}
        %
        %
        %Theorem~\ref{thm:newrule-wpsemantics}~(\ref{thm:newrule-wpsemantics-two}) and Equation~\ref{eqn:newrule-proof-casetwo-one} now yield
        %
        %
        %\begin{align*}
        %                 & \ert{\WHILEDO{\kGuard}{C}}{f} (\sigma) \\
        %       {}={}~& \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) + \wp{\WHILEDO{\kGuard}{C}}{f} (\sigma)     
        %                    \tag{by Theorem~\ref{thm:ert-wp}} \\
        %       {}={}~& 1 + \nkGuardB (\sigma) \cdot f (\sigma)
        %                    \tag{by Theorem~\ref{thm:newrule-wpsemantics}~(\ref{thm:newrule-wpsemantics-two}) and Equation~\ref{eqn:newrule-proof-casetwo-one}} \\
        %       {}={}~&  1 + \underbrace{\frac{\kGuardB (\sigma)}{1- \wp{C}{\kGuardB} (\sigma)}}_{{}={}~0 ~{}\eqcolon{}~ \frac{0}{0}} 
        %                      \cdot \left(1 + \ert{C}{0} (\sigma)
        %                    + \wp{C}{\nkGuardB \cdot f} (\sigma) \right) + \nkGuardB (\sigma) \cdot f (\sigma)~.            
        %\end{align*}
        %
        %
        %%To prove the remaining case, assume $\kGuardB (\sigma)=1$. Theorem~\ref{thm:omega-invariants} and Lemma~\ref{lem:newrule-omega-invariant} then imply
        %
        %
        %\begin{align}
        %                 & \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) \notag \\
        %        {}={}~& \lim_{n\to\infty} ~ \left( 1 + \underbrace{\kGuardB (\sigma)}_{{}={}~1} \cdot \left( \ert{C}{0} (\sigma) \cdot
        %                     \sum\limits_{i=0}^{n} \underbrace{\wp{C}{\kGuardB} (\sigma)^i}_{{}={}~1} ~+~ 
        %                     \sum\limits_{i=0}^{n-1} \underbrace{\wp{C}{\kGuardB} (\sigma)^i}_{{}={}~1} \right) \right) 
        %                     \tag{by Theorem~\ref{thm:omega-invariants} and  Lemma~\ref{lem:newrule-omega-invariant}} \\
        %        {}={}~& \lim_{n\to\infty} ~ 1 + \ert{C}{0} (\sigma) \cdot \sum\limits_{i=0}^{n} 1 ~+~\sum\limits_{i=0}^{n-1} 1
        %                     \notag \\
        %        {}={}~& \lim_{n\to\infty} ~ 1 + \ert{C}{0} (\sigma) \cdot (n+1) +n 
        %                     \notag \\
        %        {}={}~& \infty~. \label{eqn:newrule-proof-casetwo-two}  
        %\end{align}
       %
       %
       %Using Theorem~\ref{thm:ert-wp} and Equation~\ref{eqn:newrule-proof-casetwo-two}, we obtain
       %
       %
       %\begin{align*}
       %                 & \ert{\WHILEDO{\kGuard}{C}}{f} (\sigma) \\
       %        {}={}~& \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) + \wp{\WHILEDO{\kGuard}{C}}{f} (\sigma)     
       %                     \tag{by Theorem~\ref{thm:ert-wp}} \\
       %        {}={}~& \infty + \underbrace{\wp{\WHILEDO{\kGuard}{C}}{f}(\sigma)}_{{}\geq{}~ 0}
       %                     \tag{by Equation~\ref{eqn:newrule-proof-casetwo-two}} \\
       %        {}={}~& \infty \\
       %        {}={}~& 1 + \underbrace{\frac{\kGuardB (\sigma)}{1- \wp{C}{\kGuardB} (\sigma)}}_{{}={}~\infty ~{}\eqcolon{}~ \frac{1}{0}} 
       %                       \cdot \left(1 + \ert{C}{0} (\sigma)
       %                     + \wp{C}{\nkGuardB \cdot f} (\sigma) \right) + \nkGuardB (\sigma) \cdot f (\sigma)~.  \tag*{\qedhere}
       %\end{align*}
\end{proof}


==> overview.tex <==
% !TEX root = ./main.tex

\section{Overview}\label{sec:overview}

\cmcommentinline{
I recommend merging this section with the introduction as I do not think one gets a much better overview over our results here. 
Furthermore, the first new staff is currently presented on page 12. Maybe we can reduce the initial overhead a bit?
}
In this section, we give an overview of our approach by means of an example, namely the BN in Figure~\ref{fig:intro:bn}.
Our translation mechanism associates with each node in the BN a probabilistic program that we call a \emph{block}.
The blocks are then sequentially composed to a single program.
The order of blocks in the program should of course be in accordance with the dependencies in the BN.
Thus, any topological sorting of the nodes of the BN (always possible, as BNs are \emph{directed acyclic graphs}) induces a good ordering on the blocks in the BNL program.

For the BN in Figure~\ref{fig:intro:bn} with nodes $S$, $R$, and $G$, our translation yields the following blocks $B_S$, $B_R$, and $B_G$:
\begin{align*}
	B_S ~~\rhd\qquad & \IF{x_R = 0} & B_G ~~\rhd\qquad & \IF{x_S {=} 0 \wedge x_R {=} 0} \\
	%
	& \qquad \PASSIGN{x_S}{a \cdot \langle 0 \rangle + (1 - a) \cdot \langle 1 \rangle} \} \quad&& \qquad \PASSIGN{x_G}{0.01 \cdot \langle 0 \rangle + 0.99 \cdot \langle 1 \rangle} \}\\
	%
	& \ELSE \{ && \ELSE \{ ~\IF{x_S {=} 0 \wedge x_R {=} 1} \\
	%
	& \qquad \PASSIGN{x_S}{0.2 \cdot \langle 0 \rangle + 0.8 \cdot \langle 1 \rangle} \} && \qquad \PASSIGN{x_G}{0.25 \cdot \langle 0 \rangle + 0.75 \cdot \langle 1 \rangle} \}\\
	%
	&&& \ELSE \{ ~ \IF{x_S {=} 1 \wedge x_R {=} 0} \\
	%
	&~ && \qquad \PASSIGN{x_G}{0.9 \cdot \langle 0 \rangle + 0.1 \cdot \langle 1 \rangle} \}  \\
	%
	B_R ~~\rhd\qquad & \PASSIGN{x_R}{a \cdot \langle 0 \rangle + (1 - a) \cdot \langle 1 \rangle} && \ELSE \{\\
	%
	&&& \qquad \PASSIGN{x_G}{0.2 \cdot \langle 0 \rangle + 0.8 \cdot \langle 1 \rangle} \} \} \}
\end{align*}
%
%\begin{enumerate}
%	\item 
%		For node $S$ we get the block
%		%
%		\begin{align*}
%			B_S ~~\rhd\qquad & \IF{x_R = 0} \\
%			%
%			& \qquad \PASSIGN{x_S}{a \cdot \langle 0 \rangle + (1 - a) \cdot \langle 1 \rangle} \\
%			%
%			& \ELSEBRACK \\
%			%
%			& \qquad \PASSIGN{x_S}{0.2 \cdot \langle 0 \rangle + 0.8 \cdot \langle 1 \rangle} \\
%			%
%			& \}~.
%		\end{align*}
%		%
%	\item 
%		For node $R$ we get the block
%		%
%		\begin{align*}
%			B_R ~~\rhd\qquad & \PASSIGN{x_R}{a \cdot \langle 0 \rangle + (1 - a) \cdot \langle 1 \rangle}~.
%		\end{align*}
%		%
%	\item 
%		For node $G$ we get the block
%		%
%		\begin{align*}
%			B_G ~~\rhd\qquad & \IF{x_S {=} 0 \wedge x_R {=} 0} \\
%			%
%			& \qquad \PASSIGN{x_G}{0.01 \cdot \langle 0 \rangle + 0.99 \cdot \langle 1 \rangle} \\
%			%
%			& \ELSEBRACK \\
%			%
%			& \qquad \IF{x_S {=} 0 \wedge x_R {=} 1} \\
%			%
%			& \qquad \qquad \PASSIGN{x_G}{0.25 \cdot \langle 0 \rangle + 0.75 \cdot \langle 1 \rangle} \\
%			%
%			& \qquad \ELSEBRACK \\
%			%
%			& \qquad \qquad \IF{x_S {=} 1 \wedge x_R {=} 0} \\
%			%
%			& \qquad \qquad \qquad \PASSIGN{x_G}{0.9 \cdot \langle 0 \rangle + 0.1 \cdot \langle 1 \rangle} \\
%			%
%			& \qquad \qquad \ELSEBRACK \\
%			%
%			& \qquad \qquad \qquad \PASSIGN{x_G}{0.2 \cdot \langle 0 \rangle + 0.8 \cdot \langle 1 \rangle} \\
%			%
%			& \qquad \qquad \} \\
%			%
%			& \qquad \} \\
%			%
%			& \}~.
%		\end{align*}
%		%
%\end{enumerate}
%
The only topological sorting of the BN is $R$, $S$, $G$, since $G$ depends on both $S$ and $R$, and $S$ depends on $R$.
Executing $\COMPOSE{\COMPOSE{B_R}{B_S}}{B_G}$ corresponds to sampling from the BN's \emph{unconditional} joint probability distribution.

Lastly, we need to account for observation $G = 0$ and implement a rejection sampling mechanism in order to sample from the \emph{conditional} joint distribution given that $G = 0$.
The result of our translation is thus the \bnl program
%
\begin{align*}
	&\REPEAT \\
	& \qquad \COMPOSE{\COMPOSE{B_R}{B_S}}{B_G} \\
	& \UNTIL{G = 0}~.
\end{align*}
%
A static analysis of the program (i.e.\ application of our proof rule, see Theorem~\ref{thm:bnl:repeat} from p.\ \pageref{thm:bnl:repeat}) then yields that the ERT for this program is%
\footnote{A derivation of the ERT is found in Appendix~\ref{app:example:calculations}.}
%
\begin{align*}
	\frac{200 a^2 - 40 a - 460}{89 a^2 - 69 a - 21}~.
\end{align*}
%
The plot of this function is presented in \autoref{fig:intro:bn:times} (leftmost plot).
%
\begin{figure}[t]
\scalebox{.47}{
\begin{tikzpicture}
\draw[help lines, use as bounding box, white] (-1.25, -0.5) grid (7,6.2);
\begin{axis}[axis lines=middle,samples=200, xmin=0, xmax=1.1, ymin =0, ymax=350, y label style={anchor=south east}, ylabel={\LARGE time}, x label style={anchor=north west}, xlabel={\LARGE $a$}]
\addplot[thick, domain=0:1] {(200 * x^2 - 40 * x - 460)/(89 * x^2 - 69 * x - 21)};
\draw[dashed] (axis cs:0,300) -- (axis cs:1,300);
\end{axis}
\end{tikzpicture}
}
\scalebox{.47}{
\begin{tikzpicture}
\draw[help lines, use as bounding box, white] (-1, -0.5) grid (7,6.2);
\begin{axis}[axis lines=middle,samples=200, 
ymin=0, 
xmin=0, xmax=0.95, ymax=35, 
y label style={anchor=south east}, ylabel={\LARGE time}, x label style={anchor=north west}, xlabel={\LARGE $a$}]
\addplot[thick, domain=0:0.9] {(200 * x^2 - 40 * x - 460)/(89 * x^2 - 69 * x - 21)};
\draw[dashed] (axis cs:0,30.336) -- (axis cs:0.9,30.336);
\end{axis}
\end{tikzpicture}
}
\scalebox{.47}{
\begin{tikzpicture}
\draw[help lines, use as bounding box, white] (-1, -0.5) grid (7.5,6.2);
\begin{axis}[axis lines=middle,samples=200, 
ymin=0, 
xmin=0.9, xmax=1.01, ymax=350, 
y label style={anchor=south east}, ylabel={\LARGE time}, x label style={anchor=north west}, xlabel={\LARGE $a$}]
\addplot[thick, domain=0.9:1] {(200 * x^2 - 40 * x - 460)/(89 * x^2 - 69 * x - 21)};
\draw[dashed] (axis cs:0,300) -- (axis cs:1,300);
\end{axis}
\end{tikzpicture}
}
\caption{
Expected sampling times for the BN in \autoref{fig:intro:bn} when conditioning on event $G {=} 0$ plotted over different values of $a \in [0,\, 1]$.
The leftmost plot shows the expected sampling times for the whole interval $[0,\, 1]$.
The middle plot zooms in on the sampling times for $a \in [0,\, 0.9]$ and the rightmost plot for $a \in [0.9,\, 1]$.
}
\label{fig:intro:bn:times}
\end{figure}
%
The ERT of the program corresponds to the expected sampling time of the BN.

Knowing this function can be valuable.
E.g.,\ we see that the maximum is an expected sampling time of $300$ at $a=1$ and the minimum is approximately $12.86$ at $a \approx 0.4486$.
More interestingly, for large ranges of values of $a$ the BN is quite well--behaved:
For $a \in [0.08,\, 0.78]$ the expected sampling time stays below 18, i.e.\ $6\%$ of the maximum sampling time.
For $a \in [0,\, 0.89]$ it stays below 30, i.e.\ $10\%$ of the maximum, and for $a \in [0,\, 0.95]$ it still stays below 60, i.e.\ $20 \%$ of the maximum.
Above $a = 0.95$ the expected sampling time starts to grow rapidly.


==> prelim_bn.tex <==
We denote a tuple $(s_1,\ldots,s_k) \in S^{k}$ of length $k$ over some set $S$ by $\T{s}$.
Moreover, given a curried function, say $f : S \to S \to S \to S$, we often write $f(s_1,s_2,s_3)$ instead of $((f(s_1))(s_2))(s_3)$.

\begin{definition}\label{def:bayesian-network}
        A \emph{Bayesian network} is a tuple $\BN = (\NODES,\EDGES,\VALUES, \DEP,\CPTSYM)$, where
  \begin{itemize}
          \item $(\NODES,\EDGES)$ is a finite directed acyclic graph with nodes $\NODES = \{v_1,\ldots,v_n\}$ and edges $\EDGES \subseteq \NODES \times \NODES$,
          \item $\VALUES$ is a finite\cmcomment{We might drop finiteness here if we want to consider generalized Bayesian networks.} set of possible \emph{values} that can be assigned to each node,
          \item $\DEP : \NODES \To \NODES^{*}$ is a function assigning each node to the sequence of nodes (ordered by there indices) that it \emph{depends on}, i.e.
         \begin{align*}
                 \DEP(v) ~=~ v_{i_1} \ldots v_{i_m}
         \end{align*}
         with $(v_{i_j},v) \in E$, $1 \leq j \leq m$, and $i_1 < i_2 < \ldots < i_m$.
 \item $\CPTSYM$ is a function mapping each node $v \in \NODES$ to its \emph{conditional probability table} $\CPT{v}$.
         More precisely, for $k = |\DEP(v)|$, the function $\CPT{v}$ is given by a (total) function of the form
         \begin{align*}
            \CPT{v} \,:\, \underbrace{\VALUES \To \VALUES \To \ldots \To \VALUES}_{k+1~\text{times}} \To [0,1]
            \quad\text{such that}\quad    
            \sum_{z_1,\ldots,z_{k+1} \in \VALUES} \CPT{v}(z_1,\ldots,z_{k+1}) = 1.
         \end{align*}
  \end{itemize}
  The set of all Bayesian networks is denoted by $\BNS$.
\end{definition}

Each node in a Bayesian network is a (discrete) random variable.
As the name suggests, the conditional probability table $\CPTSYM$ determines the conditional probability distribution of each node $v \in \NODES$ given the nodes it depends on.
Formally, we interpret a conditional probability table as follows:
\begin{align*}
        \PROB{v=z \,|\, \DEP(v) = (z_1,\ldots,z_k)} \eeq \CPT{v}(z,z_1,\ldots,z_k)~,
\end{align*}
where $z,z_1,\ldots,z_k \in \VALUES$.

\begin{definition}
  The \emph{joint probability distribution} of a Bayesian network $\BN = (\NODES,\EDGES,\VALUES,\DEP,\CPTSYM)$ 
  with $\NODES = \{v_1,\ldots,v_n\}$ is given by 
  \begin{align*}
    \PROB{v_1,\ldots,v_n}
    \eeq \prod_{v \in \NODES} \PROB{v \,|\, \DEP(v)}
    \eeq \prod_{v \in \NODES} \CPT{v}.
  \end{align*}
\end{definition}



==> uiid.tex <==
% !TEX root = ./main.tex
\subsection{Universally Independent and Identically Distributed Loops}\label{sec:universally-iid}
%
%
%
%Our first proof rule takes a global viewpoint on the i.i.d.\ property, i.e.\ it does not depend on a particular postexpection.
%Hence, we refer to loops within this class as \emph{universally i.i.d.\ loops}.
%
%
%
\blkcommentinline{BEGIN}
\begin{definition}[Universally i.i.d.\ Loops]
       \label{def:iid}
       Let $C$ be a $\pgcl$ program and $\kGuard$ be a guard. 
       We call a loop $\WHILEDO{\kGuard}{C}$ \emph{universally independent and identically distributed} (or \emph{universally i.i.d.} for short), iff for all $f \in \E$ it holds that
       \begin{equation*}
              \wp{C}{~\iverson{\kGuard} \cdot \wp{C}{f}~} \eeq  \wp{C}{\iverson{\kGuard}} \cdot \wp{C}{f}~.
              \tag*{$\triangle$}
       \end{equation*}
\end{definition}
%\noindent
%%
%%
%%
%This defines the i.i.d.\ property in a global manner. 
The intuition is the following:
No matter which postexpectation $f \in E$ we consider, the event that the guard evaluates to true (given by $\kGuardB$) shall be uncorrelated with the expected value of $f$ (given by $\wp{C}{f}$) after one loop iteration. 
We thus require
\abovedisplayskip=0pt
\begin{align*}
	\wp{C}{~\kGuardB \cdot \wp{C}{f}~} ~{}\stackrel{!}{=}{}~ &\wp{C}{\kGuardB} \cdot \wp{C}{\wp{C}{f}} \\
	\eeq & \wp{C}{\kGuardB} \cdot \wp{\COMPOSE{C}{C}}{f}~.
\end{align*} 
\normalsize
Furthermore, executing the loop body once or twice shall yield the same expected value for $f$.
We thus require
%
\abovedisplayskip=0pt
\begin{align*}
	\wp{C}{\kGuardB} \cdot \wp{\COMPOSE{C}{C}}{f} ~{}\stackrel{!}{=}{}~ \wp{C}{\kGuardB} \cdot \wp{C}{f}~.
\end{align*}
\normalsize
%
Taking these two requirements together results in the above definition.
\blkcommentinline{END}
%
%
%
%\begin{example}
%       \label{ex:universally-iid}
%       As an example of a universally i.i.d.\ loop, consider the program in Figure~\ref{fig:circle-loop} (for some natural number $p \geq 1$ determining the precision of uniform sampling).
%       To verify this, let $f \in \E$ be an expectation and let $\rejectionProgBody$
%       denote the body of that loop. Then
%       %
%       %
%       %
%       \begin{align*}
%              &\wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \wp{\rejectionProgBody}{f}} \\
%              &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \frac{1}{121} \sum\limits_{i=0}^{10p} \sum\limits_{j=0}^{10 p} f[x/(\nicefrac i p), y/(\nicefrac j p)]}
%                      \tag{Table~\ref{table:ert}} \\
%                      &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}} \cdot \frac{1}{121} \sum\limits_{i=0}^{10p} \sum\limits_{j=0}^{10p} f[x/(\nicefrac i p), y/(\nicefrac j p)]
%              \tag{$x$ \text{and} $y$ do not occur in $f[x/i, y/j]$} \\
%              &{}={}~ \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}} \cdot  \wp{\rejectionProgBody}{f}~.
%              \tag*{$\triangle$}      
%       \end{align*}
%       %
%       %
%       %
%\end{example}
%
%
%
%\noindent
%We now derive a characterization of the $\wpsymbol$--semantics of universally i.i.d.\ loops.
%For that, we first analyze the $\wpsymbol$--semantics of their finite unrollings.
%%
%%
%%
%\begin{lemma}[$\wpsymbol$--Semantics of $n$--Unrollings of Universally I.I.D.\ Loops]
%       \label{lem:oldrule_wp_finite_approximations}
%       Let $C$ be a $\pgcl$ program and $\kGuard$ be a guard such that the loop 
%       $\WHILEDO{\kGuard}{C}$ is universally i.i.d.
%       Then, for all $n \in \Nats \setminus \{ 0 \}$ and $f \in \E$, we have
%       %
%       %
%       \abovedisplayskip=0pt
%       \begin{align*}
%              &\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} 
%              \eeq  \iverson{\kGuard} \cdot \wp{C}{\iverson{\neg \kGuard} \cdot f}
%               \cdot \left .\sum\limits_{i=0}^{n-2} \middle (\wp{C}{\iverson{\kGuard}}^i \right) + \iverson{\neg \kGuard} \cdot f~.
%       \end{align*}
%       \normalsize
%       %
%       %
%\end{lemma}
%%
%%
%%
%%
%\begin{proof}
%	By induction on $n$. See Appendix~\ref{proof-lem:oldrule_wp_finite_approximations}. \qed
%\end{proof}
%\noindent
%
%
%
%
%Using Lemma~\ref{lem:oldrule_wp_finite_approximations}, 
%This given a characterization of expected outcomes of universally i.i.d.\ loops.
%we are now in a position to establish the following theorem.
%
%
%
\blkcommentinline{BEGIN}
\begin{theorem}[$\wpsymbol$--Semantics of universally i.i.d.\ Loops] \label{thm:oldrule-wpsemantics}
       Let $C \in \pgcl$ and let $\kGuard$ be a guard.
       If $\WHILEDO{\kGuard}{C}$ is universally i.i.d., then the following two statements hold for all $f \in \E$:
       \begin{enumerate}
              \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) < 1$ it holds that
                       \label{thm:oldrule-wpsemantics-one}
                       %
                       %
                       \begin{equation*}
                              \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                              \iverson{\kGuard}(\sigma) \cdot 
                              \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
                              + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) ~.
                       \end{equation*}
                       %
                       %
               \item For all $\sigma \in \States$ with $\wp{C}{\iverson{\kGuard}}(\sigma) = 1$ it holds that
                        \label{thm:oldrule-wpsemantics-two}
                        %
                        %
                        \begin{equation*}
                        \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 
                        \nkGuardB (\sigma) \cdot f(\sigma) ~.
                        \end{equation*}
                        %
                        %
       \end{enumerate}
\end{theorem}
%
%
\begin{proof}
       The proof relies on the fact that
       %
       \begin{equation}
              \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq 
              \wp{\WHILEDO{\kGuard}{C}}{f}~,
              \label{eq:in-proof:thm:oldrule-wpsemantics}
       \end{equation}
       %
       which can easily be proven through showing by induction on $n$ that
       %
       \begin{align*}
		\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} \eeq F_f^n(0)~,
       \end{align*}
       %
       and then applying the Kleene Fixed Point Theorem.
       %, which we omit here.
       %
       \autoref{eq:in-proof:thm:oldrule-wpsemantics} is equivalent to
       \belowdisplayskip=0pt
	   \begin{equation} \label{eqn:oldrule-continuity-states}
       \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma)
        \eeq  \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma)
       \end{equation}
       \normalsize
       %
       %
       for all $\sigma \in \States$. 
       
       In order to prove the first statement of the theorem, suppose that $\wp{C}{\kGuardB}(\sigma) <1$.
       We exploit the closed form of the geometric series,
        i.e.\ $\sum_{i=0}^{\omega} q  = \sfrac{1}{1-q}$, \text{for } $|q| < 1$.
        Using this closed form, we calculate
        %
        %
        \begin{align*}
                 & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
        & \eeq  \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
                     \tag{by Equation \ref{eqn:oldrule-continuity-states}} \\
                     %
        & \eeq  \sup_{n \in \Nats}~
                      \iverson{\kGuard}(\sigma) \cdot  \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
                     \cdot \left. \sum\limits_{i=0}^{n-2} \middle( \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
                    + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
                    \tag{by Lemma \ref{lem:oldrule_wp_finite_approximations}} \\
                    %
        & \eeq   \iverson{\kGuard}(\sigma) \cdot \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
                     \cdot \left. \sum\limits_{i=0}^{\omega} \middle( \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
                    + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) \\
                    %
        & \eeq  \kGuardB (\sigma) \cdot 
                     \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}
                     + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)~. \tag{geom.\ ser.\ closed form}
        \end{align*}
        %
        %
        This proves the first statement of the theorem. 
%        
%        For the second statement of the theorem, suppose now that $\kGuardB(\sigma)=0$. 
%        We then have
%        %
%        %
%        \begin{align*}
%                 & \wp{\WHILEDO{\kGuard}{C}}{f}(\sigma) \\
%        & \eeq  \sup_{n \in \Nats}~ \wp{\WHILEDOapprox{\kGuard}{C}{n}}{f}(\sigma) 
%                     \tag{by Equation \ref{eqn:oldrule-continuity-states}} \\
%        & \eeq  \sup_{n \in \Nats}~
%                      \underbrace{\iverson{\kGuard}(\sigma)}_{{}={}0}
%                      \cdot \left( \wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)
%                      \cdot \sum\limits_{i=0}^{n-2} \wp{C}{\iverson{\kGuard}}(\sigma)^i \right) 
%                      + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma) 
%                      \tag{by Lemma \ref{lem:oldrule_wp_finite_approximations}} \\
%        & \eeq  \sup_{n \in \Nats}~ \nkGuardB(\sigma) \cdot f(\sigma) \\
%        & \eeq \nkGuardB(\sigma) \cdot f(\sigma)~.
%        \end{align*}
%        This proves the second statement of the theorem.
%        %
%        %

%
For the second statement of the theorem, suppose now that $\wp{C}{\iverson{\varphi}}(\sigma) = 1$.
We observe that this can only be true if every state $\tau$ that is reachable with non--zero probability by executing $C$ on $\sigma$ has to satisfy $\varphi$. Otherwise, the integral would not add up to exactly 1.
Formally,
%
\begin{align}
	\wp{C}{\iverson{\varphi}}(\sigma) \eeq 1 \qiff \Exp{\Sigma}{\iverson{\varphi}}{\semantics{C}{\sigma}} = 1 \qiff \forall \semantics{C}{\sigma}(\tau) > 0 \implies \iverson{\varphi}(\tau) = 1~.
	\label{eq:bennistheorem}
\end{align}
%
From that, it follows that 
%
\begin{align*}
	\wp{C}{\iverson{\neg \kGuard} \cdot f} (\sigma) \eeq \Exp{\Sigma}{\iverson{\neg \kGuard} \cdot f}{\semantics{C}{\sigma}} & \eeq \Exp{\Sigma}{f - \iverson{\kGuard} \cdot f}{\semantics{C}{\sigma}} \\
	& {\stackrel{\text{(\ref{eq:bennistheorem})}}{\eeq}} \Exp{\Sigma}{f - 1 \cdot f}{\semantics{C}{\sigma}}\\
	& \eeq \Exp{\Sigma}{0}{\semantics{C}{\sigma}} \eeq 0~.
\end{align*}
%
Now by Lemma~\ref{lem:oldrule_wp_finite_approximations}  and by $\wp{C}{\iverson{\neg \kGuard} \cdot f} (\sigma) = 0$ (see above) we get
%
\begin{align*}
	\wp{\WHILEDOapprox{\kGuard}{C}{n}}{f} (\sigma) \eeq \iverson{\kGuard}(\sigma) \cdot 0 \cdot \left .\sum\limits_{i=0}^{n-2} \middle (\ldots \right) + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)  \eeq \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)
\end{align*}
%
and thereby $\wp{\WHILEDO{\kGuard}{C}}{f} (\sigma) \eeq  \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)$.
%
%
%
\qed
\end{proof}
\blkcommentinline{END}
%\noindent
%
%
%
\blkcommentinline{BEGIN}
Verifying bounds on expected values is a very involved task.
Verifying lower bounds is even more involved in practice than upper bounds.
It is thus worthwhile to note that the characterization of Theorem~\ref{thm:oldrule-wpsemantics} does not give us only bounds on the expected values, but instead we obtain the \emph{exact} expected values.
\blkcommentinline{END}

Building on this result, we next derive the exact ERTs of universally i.i.d.\ loops.
This requires a generalization of the universally i.i.d.\ property to a fixed number of loop iterations.
%$\WHILEDO{\kGuard}{C}$. This requires the next technical lemma.
%
%
%
\begin{lemma}
      \label{lem:oldrule-technical-three}
       Let $C \in \pgcl$ and $\kGuard$ be a guard.
       If $\WHILEDO{\kGuard}{C}$ is
       universally i.i.d., then the following equation holds for all $n \in \Nats$:
       %
       %
       \begin{equation*}
              \wp{C}{\kGuardB} \cdot \wp{C}{\kGuardB}^n \eeq 
              \wp{C}{\kGuardB \cdot \wp{C}{\kGuardB}^n}~.
       \end{equation*}
       %
       %
\end{lemma}
%
%
%
\begin{proof}
       By induction on $n$. See Appendix \ref{proof-lem:oldrule-technical-three}. \qed
\end{proof}
\noindent
%
%
%
Intuitively, the above lemma ensures that the probability of the loop guard evaluating to true through one iteration is independent of the number of past iterations.
Moreover, this probability is the same for \emph{every} iteration.

In order to derive ERTs of universally i.i.d.\ loops, we provide a lower and upper $\omega$--invariant w.r.t.\  postexpectation $0$
and analyze its asymptotic behavior.
Besides being universally i.i.d., such a loop has to satisfy two additional properties:
(1) the loop body must terminate almost--surely, i.e.\ $\wp{C}{1} = 1$ and (2) every iteration runs in the same expected time. 
This is formalized by 
%
%\abovedisplayskip=0pt
\begin{align}
	\wp{C}{\ert{C}{0}} \eeq \ert{C}{0}~, \label{eq:benni:ertwp}
\end{align}
\normalsize
%
because the latter equation implies the following:
%
%
%\begin{align*}
%                           & \wp{C}{\ert{C}{0}} ~{}={}~ \ert{C}{0} \\
%       {}\Longleftrightarrow{} & \wp{C}{\ert{C}{0}} + \ert{C}{0} ~{}={}~ \ert{C}{0} + \ert{C}{0} \\
%       {}\Longleftrightarrow{} & \ert{\COMPOSE{C}{C}}{0} ~{}={}~ 2 \cdot \ert{C}{0} ~.
%                             \tag{by Theorem~\ref{thm:ert-wp} and Table~\ref{table:wp}} 
%\end{align*}
\begin{align*}
                \ert{\COMPOSE{C}{C}}{0} &~{}={}~ \ert{C}{\ert{C}{0}} \tag{by Table~\ref{table:ert}} \\
       &~{}={}~ \ert{C}{0} + \wp{C}{\ert{C}{0}} \tag{by Theorem~\ref{thm:ert-wp}} \\
       &~{}={}~ \ert{C}{0} + \ert{C}{0} \tag{by Equation \ref{eq:benni:ertwp} above}\\
       &~{}={}~ 2 \cdot \ert{C}{0}~.
\end{align*}
%
%
%
Thus, the ERT of two iterations is given by the ERT of one iteration multiplied by two. 
Notice, the fact that every iteration takes the same \emph{expected time} does not necessarily imply that every iteration needs \emph{the same} time as the following example
demonstrates.
%
%
%
\begin{example}\label{ex:same-time}
       Consider the following $\pgcl$ program:
       %
       %
       %
       \begin{align*}
             &\WHILE{x \neq 0} \\
             &\qquad \PASSIGN{x}{\frac{1}{2} \cdot \langle 0 \rangle + \frac{1}{2} \cdot \langle 1 \rangle}; \\
             &\qquad \ITE{x=0}{\COMPOSE{\SKIP}{\SKIP}}{\SKIP} \}
       \end{align*}
       %
       %
       %
       In every iteration a fair coin is tossed and--dependent on the outcome--either two or one $\SKIP$ statements are executed.
       Even though it is almost--surely not the case that every iteration runs in exactly the same time, every iteration runs in the same \emph{expected time}, namely $3.5$. \hfill $\triangle$
\end{example}
\noindent
%
%
%
%
%Having the presented preliminaries at hand, 
We are now in a position to establish our first proof rule for ERTs. %for ERTs of universally i.i.d.\ loops.
\begin{theorem}[Proof Rule for Universally I.I.D.\ Loops]
       \label{thm:oldrule-proof-rule}
       Let $C \in \pgcl$, $\kGuard$ be a guard, and $f \in E$. % be an arbitrary runtime. 
       Furthermore, assume the following conditions hold:
       %
       %
       \begin{enumerate}
              \item The loop $\WHILEDO{\kGuard}{C}$ is universally independent and identically distributed.
              \item The loop body terminates almost--surely, i.e. $\wp{C}{1} = 1$.
              \item Iterations takes the same \emph{expected} time, i.e. $\wp{C}{\ert{C}{0}} = \ert{C}{0}$.
       \end{enumerate}
       %
       %
       Then the ERT of the loop $\WHILEDO{\kGuard}{C}$ w.r.t.\  $f$ is given by:
       %
       %
       \begin{align*}
              & \ert{\WHILEDO{\kGuard}{C}}{f} \eeq 1+ \frac{\kGuardB \cdot \left(1 + \ert{C}{\nkGuardB \cdot f} \right)}{1- \wp{C}{\kGuardB}}  + \nkGuardB \cdot f~,
       \end{align*}
       %
       %
       where we define $\frac{0}{0} \coloneq 0$ and $\frac{a}{0} \coloneq \infty$ for $a \neq 0$.
\end{theorem}
%
%
\begin{proof}
       We show for every state $\sigma \in \States$ that
       %
       %
       \begin{align*}
              & \ert{\WHILEDO{\kGuard}{C}}{f}(\sigma) \eeq 1 + \frac{\kGuardB (\sigma) \cdot \left(1 + \ert{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)}  + \nkGuardB (\sigma) \cdot f (\sigma)~.
        \end{align*}
        %
        %
        To this end, we propose the following as both a lower and upper $\omega$--invariant of
        the loop
        % $\WHILEDO{\kGuard}{C}$ 
        w.r.t.\ $0$:
        %
        %
        %
        \begin{equation}\label{eqn:oldrule-proof-rule-omega-invariant}
              I_n = 1 + \kGuardB \cdot \left( \ert{C}{0} \cdot
              \sum\limits_{i=0}^{n} \wp{C}{\kGuardB}^i ~+~ 
              \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB}^i \right)
       \end{equation}
        %
        %
        %
        A check that $I_n$ is indeed a lower and upper $\omega$--invariant, is found in
        Appendix~\ref{proof-thm_oldrule-proof-rule}.
        %
        %
        %
        We now distinguish two cases for the probability of the loop guard being true after one iteration:
        %We now consider the cases 
        $\wp{C}{\kGuardB}(\sigma)<1$
        and $\wp{C}{\kGuardB}(\sigma)=1$. 
        %
        %
        \paragraph{Case $\wp{C}{\kGuardB}(\sigma)<1$:} 
        %Theorem~\ref{thm:omega-invariants}, Equation~\ref{eqn:oldrule-proof-rule-omega-invariant},
        %and the closed form of the geometric series yield
        %
        %
        \begin{align}
                         & \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) \notag \\
                {}={}~& \lim_{n\to\infty} ~ \left( 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
                             \sum\limits_{i=0}^{n} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
                             \sum\limits_{i=0}^{n-1} \wp{C}{\kGuardB} (\sigma)^i \right) \right) 
                             \tag{by Theorem~\ref{thm:omega-invariants} and  Equation~\ref{eqn:oldrule-proof-rule-omega-invariant}} \\
                {}={}~& 1 + \kGuardB (\sigma) \cdot \left( \ert{C}{0} (\sigma) \cdot
                             \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i ~+~ 
                             \sum\limits_{i=0}^{\infty} \wp{C}{\kGuardB} (\sigma)^i \right) 
                             \notag \\
                 {}={}~& 1 + \kGuardB (\sigma) \cdot \left( 
                               \frac{\ert{C}{0} (\sigma)}{1-\wp{C}{\kGuardB} (\sigma)} + 
                                \frac{1}{1-\wp{C}{\kGuardB} (\sigma)} \right)      
                                \tag{geometric series} \\
                 {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 
                               \ert{C}{0} (\sigma) + 1 \right)}{1-\wp{C}{\kGuardB} (\sigma)}~. 
                               \label{eqn:oldrule-proof-caseone}                                                                    
        \end{align}
        %
        %
        Now, by Theorem~\ref{thm:ert-wp}, Theorem~\ref{thm:oldrule-wpsemantics}~(\ref{thm:oldrule-wpsemantics-one}), and Equation~\ref{eqn:oldrule-proof-caseone}, we obtain
        %
        %
        \begin{align*}
                         & \ert{\WHILEDO{\kGuard}{C}}{f} (\sigma) \\
               {}={}~& \ert{\WHILEDO{\kGuard}{C}}{0} (\sigma) + \wp{\WHILEDO{\kGuard}{C}}{f} (\sigma)   
                            \tag{by Theorem~\ref{thm:ert-wp}} \\
               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 
                            \ert{C}{0} (\sigma) + 1 \right)}{1-\wp{C}{\kGuardB} (\sigma)} +
                            \iverson{\kGuard}(\sigma) \cdot 
                            \frac{\wp{C}{\iverson{\neg \kGuard} \cdot f}(\sigma)}{1-\wp{C}{\iverson{\kGuard}}(\sigma)}  + \iverson{\neg \kGuard}(\sigma) \cdot f(\sigma)
                            \tag{by Theorem~\ref{thm:oldrule-wpsemantics}~(\ref{thm:oldrule-wpsemantics-one}) and Equation~\ref{eqn:oldrule-proof-caseone}} \\
               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 1 + \ert{C}{0} (\sigma)
                            + \wp{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)} 
                             + \nkGuardB (\sigma) \cdot f (\sigma)\\
               {}={}~& 1 + \frac{\kGuardB (\sigma) \cdot \left( 1 + \ert{C}{\nkGuardB \cdot f} (\sigma) \right)}{1- \wp{C}{\kGuardB} (\sigma)}  + \nkGuardB (\sigma) \cdot f (\sigma)~. \tag{by Theorem~\ref{thm:ert-wp}}                                  
        \end{align*}
        %
        %
        
        \paragraph{Case $\wp{C}{\kGuardB} (\sigma)=1$:} For a formal consideration of this case we again refer to Appendix~\ref{proof-thm_oldrule-proof-rule}. 
        Intuitively, if $\wp{C}{\kGuardB} (\sigma)=1$, the loop guard is almost--surely true after an execution of the loop body on initial state $\sigma$.
        Hence, the ERT of the loop is infinite if it is executed at least once.
        Otherwise, it is $1$ due to the first (and only) guard evaluation.
        %The reason is that $\wp{C}{\kGuardB} (\sigma)$ denotes the probability of the guard evaluating to $\true$ after one iteration on initial state $\sigma$. 
        %That is, if
        %$\wp{C}{\kGuardB} (\sigma) = 1$, then the guard evaluates to $\true$ after \emph{every} iteration.
        %Here we provide a sketch:
       % Since $\wp{C}{\kGuardB} (\sigma)$ denotes the probability of the loop guard evaluating to $\true$ after one iteration, $\wp{C}{\kGuardB} (\sigma)=1$
       % implies that the guards evaluates to $\true$ after \emph{every} iteration. Thus, if the initial state satisfies the guard (i.e.\ $\kGuardB$).
       \qed
\end{proof}
%
%
%
%Let us demonstrate how Theorem~\ref{thm:oldrule-proof-rule} to a given i.i.d.\ loop in the next example.
%
%
%
%\newcommand{\exIIDLoop}{L}
%\newcommand{\exIIDLoopBody}{L_{\mathit{body}}}
%\begin{example}
%       Consider the following i.i.d.\ loop $\exIIDLoop$ and let $\exIIDLoopBody$ denote its body.
%       %
%       %
%       %
%       \begin{align*}
%              &\WHILE{i > 6} \\
%              &\qquad \PASSIGN{a_0, a_1, a_2}{\frac{1}{2} \cdot \langle 0 \rangle  + \frac{1}{2} \cdot \langle 1 \rangle}; \\
%              &\qquad \ASSIGN{i}{4a_2 + 2a_1 + a_0 + 1} \\
%              &\}
%       \end{align*}
%       %
%       %
%       %
%      The loop simulates a fair die by means of three fair toin cosses. We want to determine $\ert{L}{0}$, i.e. the average amount of guard evaluations and assignments necessary
%      to simulate the die, by applying Theorem~\ref{thm:oldrule-proof-rule}. We omit the calculations verifying that the premises of the theorem hold, which is relatively straightforward.
%      We have 
%       $\wp{\exIIDLoopBody}{\iverson{i > 6}} = \sfrac{1}{4}$ and $\ert{\exIIDLoopBody}{0} = 4$ due to the four assignments. Thus, we obtain
%       %
%      %
%      \begin{align*}
%                       &\ert{L}{0} \\
%                       &{}={}~ 1 + \frac{\iverson{i > 6}}{1 - \wp{\exIIDLoopBody}{\iverson{i > 6}}} \cdot \left(1 + \ert{\exIIDLoopBody}{0} \right)
%              ~{}={}~ 1 + \frac{\iverson{i > 6}}{1 - \sfrac{1}{4}} \cdot \left(1 + 4 \right) ~{}={}~ 1 + \iverson{i > 6} \cdot \frac{20}{3}~.
%       \end{align*}
%       %
%       %
%       %
%       Consequently, if $i > 6$ holds before the loop is executed, its ERT is  $1 + \sfrac{20}{3} \approx 7.67$. \hfill $\triangle$
%\end{example}
%
%
%
\begin{example}
        Let us determine the ERT of our running example --- the $\pgcl$ program $\rejectionProg$ from Figure~\ref{fig:circle-loop}. 
        We have already verified that $\rejectionProg$ is universally i.i.d.\ in Example~\ref{ex:universally-iid}. Since the loop body, denoted $\rejectionProgBody$, is loop--free,
        it holds that $\wp{\rejectionProgBody}{1}=1$. 
        Furthermore it is straightforward to verify that every iteration runs in the same expected time, i.e. $\wp{\rejectionProgBody}{\ert{\rejectionProgBody}{0}} = \ert{\rejectionProgBody}{0}$. 
        %Verifying this is straightforward and omitted here. 
        Consequently, Theorem~\ref{thm:oldrule-proof-rule} is applicable. 
        Hence,
        %
        %
        %
        \belowdisplayskip=0pt
         \begin{align}\label{eqn:ex-universally-iid-runtime}
              \ert{\rejectionProg}{0}
              ~{}={}~ 1+ \frac{\iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \left(1 + \ert{\rejectionProgBody}{0} \right)}{1- \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}}~,
       \end{align}
       \normalsize
        %
        %
        %
        where
        %
        %
        %
        \begin{equation*}
               \wp{\rejectionProgBody}{\iverson{(x-5)^2 + (y-5)^2 \geq 25}}
              ~{}={}~ \frac{48}{121}
              \qquad \text{and} \qquad \ert{\rejectionProgBody}{0} ~{}={}~ 2~.
              \tag{by Table~\ref{table:wp} and Table~\ref{table:ert}}            
        \end{equation*}
        %
        %
        %
        By plugging the above values into Equation~\ref{eqn:ex-universally-iid-runtime}, we obtain the exact ERT of $\rejectionProg$:
        %
        %
        %
        \begin{equation*}
               \ert{\rejectionProg}{0} ~{}={}~ 1 + \iverson{(x-5)^2 + (y-5)^2 \geq 25} \cdot \frac{363}{73}
        \end{equation*}
        %
        %
        %
        Hence $1 + \sfrac{363}{73} \approx 5.97$ guard evaluations and probabilistic assignments are required on average to sample a
        point within the circle uniformly at random using the rejection sampling method.\hfill $\triangle$
\end{example}
%
%
%
